Bayesian decision-making under misspecified priors with applications to meta-learning

Thompson sampling and other Bayesian sequential decision-making algorithms are among the most popular approaches to tackle explore/exploit trade-offs in (contextual) bandits. The choice of prior in these algorithms offers flexibility to encode domain knowledge but can also lead to poor performance when misspecified. In this paper, we demonstrate that performance degrades gracefully with misspecification. We prove that the expected reward accrued by Thompson sampling (TS) with a misspecified prior differs by at most $\tilde{\mathcal{O}}(H^2 \epsilon)$ from TS with a well specified prior, where $\epsilon$ is the total-variation distance between priors and $H$ is the learning horizon. Our bound does not require the prior to have any parametric form. For priors with bounded support, our bound is independent of the cardinality or structure of the action space, and we show that it is tight up to universal constants in the worst case. Building on our sensitivity analysis, we establish generic PAC guarantees for algorithms in the recently studied Bayesian meta-learning setting and derive corollaries for various families of priors. Our results generalize along two axes: (1) they apply to a broader family of Bayesian decision-making algorithms, including a Monte-Carlo implementation of the knowledge gradient algorithm (KG), and (2) they apply to Bayesian POMDPs, the most general Bayesian decision-making setting, encompassing contextual bandits as a special case. Through numerical simulations, we illustrate how prior misspecification and the deployment of one-step look-ahead (as in KG) can impact the convergence of meta-learning in multi-armed and contextual bandits with structured and correlated priors.

==> body/Gaussian_model.tex <==
%!TEX root = ../main.tex
\newcommand{\calN}{\mathcal{N}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\nn}{\nonumber}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\detst}{\det_{\star}}

\section{New formulation}
\begin{align*}
    & \pi_\theta = \arg\max_{\pi\in\Pi} R(\theta;\pi)\\
& \textrm{Thompson sampling: } \Pi = \{ \pi_{\textrm{TS},\theta} : \theta \in \Theta \}\\
& \textrm{Sensitivity:} \sup_{\pi \in \Pi} |R(\theta;\pi) - R(\theta';\pi)| \leq d(\theta,\theta') 
\end{align*}

We actually need
\begin{align*}
    R(\theta;\pi_\theta) - R(\theta; \pi_{\theta'}) \leq d(\theta,\theta') 
\end{align*}
\section{Analyzing Likelihoods: Gaussian Case}
We found that using naive averaging yields biased estimates of underlying parameters. Let us show how MLE computation circumvents this hindrance.

\subsection{Simple Setting}
Consider a simple scalar setting with a single arm. For a fixed parameter $\mu \in \R$, each episode proceeds as follows
\begin{itemize}
	\item  An episode mean $\theta$ is drawn via $\theta \sim \calN(\mu,\sigma_{0}^2)$. 
	\item $x_{1},\dots,x_{\tau}$ samples are drawn as $x_i \sim \calN(\theta,\sigma^2)$. Here, $\tau$ is a stopping time with respect to the natural filtration. 
\end{itemize}
Let us compute the relevant log likelihood:
\begin{lemma}\label{lem:likelihood_comp} Fix a sequence $x_{1},\dots,x_\tau$. Then, the likelihood function $p(x_{1:n} \mid \mu)$ satisfies
\begin{align*}
\log p(x_{1:\tau} \mid \mu) = \frac{1}{2\sigma_0^2}\left(\mu^2 - 2\mu \xbar_{\tau}\right)\left(1 - \sigma_{\tau}^2 \right)  + C(\tau,x_{1:\tau}).
\end{align*}
where $C: \N \times \R^{*} \to \R$ does not depend on $\mu$, and $\xbar_{\tau}$ is the empirical mean, and $\sigma_{\tau}^2 = \frac{\sigma^2}{\sigma_0^2\tau + \sigma^2}$. 
\end{lemma}
The above lemma shows that the likelihood function, up to scaling and additive constants independent of $\mu$, has the form $f(\mu) := \left(\mu^2 - 2\mu \xbar_{\tau}\right)\cdot\left(1 - \sigma_{\tau}^2\right)$. The left hand side is minimized by setting $\mu = \xbar_{\tau}$. But, if we take the expectations, we see that the population MLE is 
\begin{align*}
\mu^{\mathrm{MLE}} := \argmin_{\mu} \E[f(\mu)] \gets \frac{\E[\xbar_{\tau}\left(1 - \sigma_{\tau}^2 \right) ]}{ \E[\left(1 - \sigma_{\tau}^2 \right)]}
\end{align*}
This is quite surpsing. By the consistency of the MLE, it follows that $\mu^{\mathrm{MLE}} = \mu$! In other words, 
\begin{align*}
\mu = \frac{\E[\xbar_{\tau}\left(1 - \sigma_{\tau}^2 \right) ]}{ \E[\left(1 - \sigma_{\tau}^2 \right)]}
\end{align*}



Indeed, consider $n$ episodes with data and stopping times $(x_{1:\tau^{(i)}}^{(i)},\tau^{(i)})_{1 \le i \le n}$. Then, the estimator
\begin{align*}
\widehat{\mu} = \frac{\sum_{i=1}^n \xbar_{\tau^{(i)}}^{(i)}\left(1 - \sigma_{\tau^{(i)}}^2 \right)}{\sum_{i=1}^n \left(1 - \sigma_{\tau^{(i)}}^2 \right)}
\end{align*}
is a consistent estimator of $\mu$! thus, we find that the MLE gives rise to a weighting scheme that gives consistent estimates. 

\subsection{Full Dimensional Setting}

\begin{lemma} Let $S = (X_{a_i},a_i)_{1 \le i \le H}$ denote a sample, let $\tau = (\tau_1,\dots,\tau_A)$ denote the vector of number of times each coordinate is sampled, and let $D :=  \frac{\diag(\tau_i)}{\sigma^2}$. Then, 
\begin{align*}
-2\log p(S \mid \mu,\Sigma) = \log(\det I + \Sigma D) + \|\xbar-\mu\|_{B}^2, 
\end{align*}
where we have defined $B := D - D(D + \Sigma^{-1})^{-1} D$.
\end{lemma}
\subsection{Higher Dimensions}


Let $S = (X_{a_i},a_i)_{1 \le i \le H}$ denote a sample.  Let
$\tau = (\tau_1,\dots,\tau_A)$ denote the vector of number of times each coordinate is sampled. Let $D :=  \frac{\diag(\tau_i)}{\sigma^2}$, and $\Lambda = \Sigma^{-1}$. Given a symmetric matrix $A \succeq 0 $, we let $\detst(A) := \prod_{i:\lambda_i(A) > 0}\lambda_i(A)$. We have
\begin{align}
p(S \mid \mu,\Sigma) &= \int_{\theta \in \R^d} p(S,\theta \mid \mu,\Sigma)\rmd \theta\nn\\
%
&= \tfrac{1}{\sqrt{\detst(2\pi D^{\dagger}) \det(2\pi\Sigma) }} \int_{\theta \in \R^d}  e^{- \frac{1}{2}\|\theta - \xbar\|_{D}^2 - \frac{1}{2}\| \theta - \mu \|^2_{\Lambda}}\rmd \theta\nn\\
%
&= \tfrac{1}{\sqrt{\detst(2\pi D^{\dagger}) \det(2\pi\Sigma) }} \int_{\theta \in \R^d}  e^{- \frac{1}{2}\left( \|\theta\|_{D + \Lambda}^2 + 2 \langle \theta, D \xbar + \Lambda \mu \rangle +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 \right)}\rmd \theta\nn\\
&= \tfrac{1}{\sqrt{\detst(2\pi D^{\dagger}) \det(2\pi\Sigma) }} \int_{\theta \in \R^d}  e^{- \frac{1}{2}\left( -\|\theta - (D+\Lambda)^{-1}(D\xbar + \Lambda \mu)\|_{D + \Lambda}^2 - \|(D\xbar + \Lambda \mu)\|_{(D+\Lambda)^{-1}}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 \right)}\rmd \theta \nn\\
&= \frac{e^{- \frac{1}{2}\left(\|(D\xbar + \Lambda \mu)\|_{(D+\Lambda)^{-1}}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 \right)}}{\sqrt{\detst(2\pi D^{\dagger}) \detst(2\pi\Sigma) }} \int_{\theta \in \R^d}  e^{- \frac{1}{2} \left(\|\theta - (D+\Lambda)^{-1}(D\xbar + \Lambda \mu)\|_{D + \Lambda}^2\right) }\rmd \theta \label{eq:some_integral}
\end{align}
We can evaluate the right-most integral via
\begin{align*}
\int_{\theta \in \R^d}  e^{- \frac{1}{2} \|\theta - (D+\Lambda)^{-1}(D\xbar + \Lambda \mu)\|_{D + \Lambda}^2 }\rmd \theta &= \int_{\theta \in \R^d}  e^{- \frac{1}{2} \|\theta \|_{D + \Lambda}^2 }\rmd \theta\\
&= \sqrt{\det(2\pi(D+\Lambda)^{-1})} = \sqrt{\det(2\pi (D+ \Sigma^{-1})^{-1})}
\end{align*}
Hence, 
\begin{align*}
p(S \mid \mu,\Sigma) &= \tfrac{\sqrt{\det(2\pi(D+\Sigma^{-1})^{-1})}}{\sqrt{\detst(2\pi D^{\dagger}) \det(2\pi\Sigma) }}e^{- \frac{1}{2}\left(-\|(D\xbar + \Lambda \mu)\|_{(D+\Lambda)^{-1}}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 \right)}\\
&= \tfrac{1}{\sqrt{\detst(2\pi D^{\dagger}) \det(\Sigma (D+\Sigma^{-1})) }}e^{- \frac{1}{2}\left(-\|(D\xbar + \Lambda \mu)\|_{(D+\Lambda)^{-1}}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 \right)}\\
&= \tfrac{1}{\sqrt{\detst(2\pi D^{\dagger}) \det(I + \Sigma D)}}e^{- \frac{1}{2}\left(-\|(D\xbar + \Lambda \mu)\|_{(D+\Lambda)^{-1}}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 \right)}
\end{align*}
Set $A = (D+\Lambda)^{-1}$. Then, 
\begin{align}
-\|(D\xbar + \Lambda \mu)\|_{A}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 &= \|\mu\|_{\Lambda - \Lambda A \Lambda}^2 + \|\xbar\|_{D - DAD}^2 - 2 \langle \Lambda \mu, A D \xbar \rangle \label{eq:some_sub}
\end{align}
Now, set
\begin{align}
B &:= \Lambda - \Lambda A \Lambda\nn\\
&= \Lambda ( I - A \Lambda) = \Lambda ( I - (\Lambda+D)^{-1} \Lambda )\nn\\
&= \Lambda ( I - A \Lambda) = \Lambda ( I - (\Lambda+D)^{-1} (\Lambda + D) + (\Lambda + D)^{-1}D )\nn\\
&= \Lambda ( I - I + A \Lambda) = \Lambda A D. \label{eq:lamad}
\end{align}
Since $B,\Lambda,A,D$ are all symmetric,
\begin{align*}
B = (\Lambda A D)^\top = D A \Lambda =  D - D A D,
\end{align*}
where the last line follows from mirroring the computation in the simplification of $B$ (\Cref{eq:lamad}).  Hence, subsituting in \Cref{eq:some_sub},
\begin{align*}
-\|(D\xbar + \Lambda \mu)\|_{A}^2  +  \|\mu\|_{\Lambda}^2 + \|\xbar\|_{D}^2 &= \|\mu\|_{B}^2 + \|\xbar\|_{B}^2 - 2 \langle B \mu,  \xbar \rangle = \|\mu - \xbar\|_{B}^2. 
\end{align*}
Thus, using $B = D - DAD$ as our definition of $B$ (which is equivalent to the others above),
\begin{align*}
p(S \mid \mu,\Sigma) &= \tfrac{1}{\sqrt{\detst(2\pi D^{\dagger}) \det(I + \Sigma D)}}e^{- \frac{1}{2}\|\xbar - \mu\|_{B}^2} \propto \det(I + \Sigma D)^{1/2}e^{- \frac{1}{2}\|\xbar - \mu\|_{B}^2} 
\end{align*}
\newcommand{\calV}{\mathcal{V}}
Finally, let simplify, and thus
\begin{align*}
2\log p(S \mid \mu,\Sigma) = -\log(\det I + \Sigma D) - \|\xbar-\mu\|_{B}^2.
\end{align*}
Finally, set $B = D - D(D + \Sigma^{-1})^{-1} D$.


\subsection{Proof of \Cref{lem:likelihood_comp}}
\begin{proof}
Since $\tau$ is a stopping time, it is entirely determined by the likelihoods of $x_{1:\tau}$. Hence, we can write
\begin{align*}
p(x_{1:\tau} \mid \mu) &= \int_{\theta \in \R} p(x_{1:\tau} \mid \theta)p(\theta \mid \mu)\rmd \theta\\
&= \int_{\theta} \frac{1}{(2\pi)^{(1+\tau)/2}}\exp\left(\frac{1}{2\sigma^2}\sum_{t=1}^{\tau} (x_t - \theta)^2  + \frac{1}{2 \sigma_{0}^2}(\theta - \mu)^2 \right) \rmd \theta. 
\end{align*}
Let us simplify the exponent. Set $\xbar_\tau := \frac{1}{\tau}\sum_{i=1}^\tau x_t$, 
\begin{align*}
\frac{1}{\sigma^2}\sum_{t=1}^{\tau} (x_t - \theta)^2  + \frac{1}{ \sigma_{0}^2}(\theta - \mu)^2 &=  \left(\frac{\tau  }{\sigma^2} + \frac{\mu}{\sigma_0^2}\right)\theta^2   -2\theta\left(\frac{\tau \xbar_{\tau} }{\sigma^2} + \frac{\mu}{\sigma_0^2}\right) \theta + \frac{\mu^2}{\sigma_0^2} +\underbrace{\frac{1}{\sigma^2}\sum_{t=1}^{\tau}x_t^2}_{:= C_1(x_{1:\tau})} 
\end{align*} 
Introduce further shorthand $n_{\tau} :=\left(\frac{\tau  }{\sigma^2} + \frac{1}{\sigma_0^2}\right) $, and $\ybar_{\tau} = \frac{\tau \xbar_{\tau} }{\sigma^2} + \frac{\mu}{\sigma_0^2}$. Completing the square gives
\begin{align*}
\frac{1}{\sigma^2}\sum_{t=1}^{\tau} (x_t - \theta)^2  + \frac{1}{ \sigma_{0}^2}(\theta - \mu)^2 &=  n_{\tau}\theta^2  -2\theta \ybar_{\tau}   + \frac{\mu^2}{\sigma_0^2} +C_1(x_{1:\tau})\\
&=  n_{\tau}(\theta  -\ybar_{\tau}/n_{\tau})^2  - \frac{\ybar_{\tau}^2}{n_{\tau}}  + \frac{\mu^2}{\sigma_0^2} +C_1(x_{1:\tau})
\end{align*} 
Finally, we may simplify 
\begin{align*}
\frac{\ybar_{\tau}^2}{n_{\tau}} = \frac{2\mu \tau \xbar_{\tau}}{\sigma^2 \sigma_0^2 n_{\tau}} + \frac{\mu^2}{\sigma_0^4 n_{\tau}} + C_2(x_{1:\tau})
\end{align*}
Setting $2C_{3}(x_{1:\tau}) = C_1(x_{1:\tau}) + C_{2}(x_{\tau})$, we find
\begin{align*}
\frac{1}{2\sigma^2}\sum_{t=1}^{\tau} (x_t - \theta)^2  + \frac{1}{2 \sigma_{0}^2}(\theta - \mu)^2 =  \frac{1}{2} n_{\tau}(\theta  -\ybar_{\tau}/n_{\tau})^2  + \underbrace{\frac{\mu^2}{2\sigma_0^2}(1 - \frac{1}{\sigma_0^2 n_{\tau}}) - \frac{\mu \tau \xbar_{\tau}}{\sigma^2 \sigma_0^2 n_{\tau}}}_{:= f(\mu,x_{1:\tau})} + C_{3}(x_{1:\tau})
\end{align*}
Hence, computing the Gaussian integral up to normalizing constants (which, depends only on $\tau$)
\begin{align*}
\log p(x_{1:\tau} \mid \mu) = f(\mu,x_{1:\tau}) +  C_{3}(x_{1:\tau}) +  c(\tau),
\end{align*}
where the normalizing constants depends only on $\tau$. Since $\tau$ is a stopping time, it depends only on $x_{1:\tau}$. Thus, we are left with
\begin{align*}
\log p(x_{1:\tau} \mid \mu) &= \frac{\mu^2}{2\sigma_0^2}(1 - \frac{1}{\sigma_0^2 n_{\tau}}) - \frac{\mu \tau \xbar_{\tau}}{\sigma^2 \sigma_0^2 n_{\tau}} + C(\tau,x_{1:\tau})\\
&= \frac{\mu}{2\sigma_0^2}\left(\mu\left(1 - \frac{1}{\sigma_0^2 n_{\tau}}\right) - \frac{\tau \xbar_{\tau}}{\sigma^2 n_{\tau}}\right) + C(\tau,x_{1:\tau}).
\end{align*}
Let us simplify
\begin{align*}
\frac{\tau}{\sigma^2 n_{\tau}} = \frac{\tau}{\tau + \sigma^2/\sigma_0^2} = 1 - \frac{\sigma^2/\sigma_0^2}{\tau + \sigma^2/\sigma_0^2} = 1-  \frac{\sigma^2}{\sigma_0^2\tau + \sigma^2}
\end{align*}
Similarly,
\begin{align*}
\frac{\sigma^2}{\sigma_0^2 n_{\tau}} = \frac{\sigma^2}{\sigma_0^2 \tau/\sigma^2 n_{\tau} + 1} = \frac{\sigma^2}{\sigma_0^2\tau + \sigma^2}
\end{align*}
THus,
\begin{align*}
\log p(x_{1:\tau} \mid \mu) &= \frac{\mu^2}{2\sigma_0^2}(1 - \frac{1}{\sigma_0^2 n_{\tau}}) - \frac{\mu \tau \xbar_{\tau}}{\sigma^2 \sigma_0^2 n_{\tau}} + C(\tau,x_{1:\tau})\\
&= \frac{1}{2\sigma_0^2}\left(\mu^2 - 2\mu \xbar_{\tau}\right)\left(1 - \frac{\sigma^2}{\sigma_0^2\tau + \sigma^2}\right)  + C(\tau,x_{1:\tau}).
\end{align*}

\end{proof}


==> body/checklist.tex <==
%!TEX root = ../neurips_main.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
\begin{comment}
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
  \end{comment}
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We describe in discussion the limitations to $n$-Monte Carlo algorithms, computational challenges of sampling, and statistical challenges in estimating complex priors.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{ See, e.g. \Cref{defn:n_monte_carlo}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Yes, in the supplement.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplement for code, and Appendix A for experimental details.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See supplement for code, and Appendix A for experimental details.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{see, e.g. Figure 1.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, see Appendix A in supplement.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> body/explore-first.tex <==




\section{Story}
Par. 1: Bayesian decision making algorithms are ubiquitous in various disciplines because they allow us to encode strong inductive biases through priors. 

not well understood of how well they adapt to mis-specifications

Par. 2: A concrete setting  where mis-specification is inherent is in meta-learning... 

Thompson Sampling is myopic

generic sensitivity bound that bounds...


\begin{itemize}
    \item Introduction
    \begin{itemize}
        \item Motivation: Thompson sampling and other Bayesian algorithms are popular across many applications. Prior is a powerful feature: allows transfer learning, meta-learning, other forms of prior knowledge. The key question: how to learn the prior and what's the impact of misspecification.
        \item Contributions
        \begin{itemize}
            \item Sensitivity bound for TS. Applies to a wider class of Bayesian algorithms.
            \item Generic meta-learning algorithm, also applicable to other Bayesian base algorithms.
        \end{itemize}
    \end{itemize}
\end{itemize}


\akcomment{Comments about non-robust algorithms and our assumptions about what Bayesian algorithms we can handle. I think it would be illuminating to have an example of a highly non-robust algorithm (to motivate assumptions?).  }


\section{Explore-first approach}

This note is based on the paper \cite{vinayak2019maximum} and the discussion on February 3rd.

Setup:
\begin{itemize}
  \item There are $K$ arms and the reward model is Bernoulli.

  \item We assume that we can force the base learner to do some uniform exploration in the first several rounds of any given meta-round.

\end{itemize}

In the $i$-th meta-round, a $[0,1]^K$-valued random vector $\vec\mu_i$ is drawn independently from an unknown distribution $P^*$, and the base learner engages in the bandit problem for $H$ steps with mean rewards specified by $\vec\mu_i$.

In each of the first $N$ meta-rounds, we force the base learner to cycle through the $K$ arms in the first $tK$ steps.
So, from each such meta-round $i$, we have independent draws from $\operatorname{Bin}(\mu_i(a), t)$ for each $a = 1,\dotsc,K$
(The numbers $t$ and $N$ will be specified shortly.)
We call this the exploration data, which we'll use to estimate $P^*$.

The theorem of \cite{vinayak2019maximum} says that for any $N$, if
\begin{equation*}
  t \in [ \Omega(\log N), O(N^{\frac29-\epsilon}) ] ,
\end{equation*}
there is an estimator $\hat P$ based on the exploration data through $N$ meta-rounds of $P^*$ that is accurate up to $W_1$-distance of
\begin{equation*}
  O\left( \frac1{\sqrt{t \log N}} \right) .
\end{equation*}

Question:
\begin{quote}
  If we have an $\delta$-accurate estimate of $P^*$ (in $W_1$-distance), what is the (ex-post) regret over the $H$ rounds of Thompson sampling based on this estimate?
\end{quote}
We assume the answer to this question is $O(\delta H)$.

The explore-first meta-algorithm is as follows.
We do the pure exploration of each arm $t$ times per each of the first $N$ meta-rounds, after which we form an estimate of $P^*$ and then supply it to Thompson sampling for the remaining meta-rounds.

The regret after $T$ meta-rounds is
\begin{equation*}
  HN + O\left( \frac{H(T-N)}{\sqrt{t \log N}} \right)
\end{equation*}
Further assuming $H \geq K N^{0.2}$, we can set $t = N^{0.2}$ and $N = T^{10/11}$ so that the regret becomes
\begin{equation*}
  O\left( HT^{10/11} \right) .
\end{equation*}
(I have ignored log factors.)


\section{Low rank MDP calculations}
Let us consider the MDP approach for meta-learning, and let us assume that the the prior is supported on $M$ bandit instances parameterized by $\mu_1,\ldots,\mu_M$. Therefore, the set of possible priors is
\begin{align*}
    \mathcal{P} := \left\{ \sum_i \theta_i P_{\mu_i} : \theta \in \Delta(M) \right \} 
\end{align*}
Here $P_{\mu_i}$ is the "bandit" distribution parameterized by $\mu_i$. We assume that $\mu_1,\ldots,\mu_M$ are known and only $\theta$ is unknown to the learner. 

For the MDP, we define the state space to be the entire history of interaction, that is all actions taken and all rewards collected so far in this episode. We will simply call these objects $s$. 
\begin{proposition}
If the prior distribution is $\theta$ then the transition operator satisfies
\begin{align*}
    T_\theta (s' | s, a) = \sum_{i=1}^M P_\theta(\mu_i | s)\cdot P_{\mu_i}(s'|s,a)
\end{align*}
Here $P_{\theta}(\mu_i | s)$ is the posterior distribution given the history $s$ and $P_{\mu_i}$ is the "one-step" transition operator given that the parameters are $\mu_i$. 
\end{proposition}
This is \emph{almost} the low rank MDP structure, but unfortunately the current state $s$ appears in both terms. This is highly problematic. On the other hand, if we can show that
\begin{align*}
    P_\theta(\mu_i | s) = \phi(s)^\top g_i(\theta),
\end{align*}
for some known functions $\phi,g_i$ then we would be in the "linearly-combined models" setting, for which sample-efficiency is information theoretically possible. 

==> body/mdp_approach.tex <==
\section{The MDP approach}
Consider the bernoulli setting, where there is some prior $\mu$ over parameter $\vec{p} \in [0,1]^K$ and in each meta-round: (a) parameter $\vec{p}_t \sim \mu$ is drawn, (b) learner interacts with a Bernoulli bandit with arms parametrized by $\vec{p}_t$. 

We re-formulate each meta-round as a single episode of a POMDP as follows: (a) The (hidden) state is $\vec{p}_t$, and the starting state distribution is $\mu$, (b) the latent transition operator is degenerate, so the agent remains in the same state for the entire episode, (c) there are no observations, (d) the reward is sampled from $\textrm{Ber}(p(a))$ when taking action $a$ in hidden state $\vec{p}$.

As is standard, we can re-express this POMDP as an MDP on the history of interaction, which is naively $((a_1,r(a_1), \ldots, a_{h-1},r(a_{h-1})$ at time $h$. Due to the fact that the hidden states does not change over time, the time steps when we play each action in the history is not relevant. Therefore we can summarize the history concisely as $\{(N_{h-1}(a), R_{h-1}(a))\}_{a \in [K]}$ where $N_{h-1}(a)$ is the number of times we have played action $a$ and $R_{h-1}(a) = \sum_{i=1}^{h-1}\one\{a_i = a\} r_i$ is the cumulative reward for these pulls. Since these $2K$ statistics take values in $\{0,H-1\}$, we see that we have a "tabular" MDP with $O(H^{2K})$ states and $K$ actions per state. 

By a standard MDP regret analysis, we can get
\begin{align*}
    \sum_{t=1}^T V^\star - V^{\pi_t} \leq \tilde{O}(H\sqrt{H^{2K}KT} + H^{2(K+1)}K\log(T))
\end{align*}
over $T$ meta-rounds.

Note that $V^\star$ is the optimal policy that knows the prior $\mu$, but does not know the draw $\vec{p}_t$ at the beginning of each episode. This corresponds to the optimal, non-myopic, Bayesian algorithm for the bandit problem with prior $\mu$.

\paragraph{Todo.}
\begin{enumerate}
    \item Make the "sufficient statistic" argument precise?
    \item Compare to Thompson sampling? Either by comparing benchmarks or by using the complexity of the prior somehow?
    \item Can we shrink the state space here to go beyond Bernoulli? We would have to do some coarsening or "state abstraction" and then incur some approximation error. 
\end{enumerate}

\section{Lower bounds on the MDP approach}

We will show that MDP learning in the meta-learning Bernoulli setup requires an exponential number of meta-rounds in the number of arms. To do this, we will consider a family of priors with `information revealing' arms, whose biases encode the location of the best arm. Specifically, each prior will be indexed by a function $f: \{0,1 \}^m \rightarrow [K]$, and will be a distribution over $m + K$-dimensional bias vectors. For a function $f$, the corresponding prior is $\mu_f$ generates a bias vector as follows:
\begin{itemize}
	\item Draw $(X_1, \ldots, X_m) \sim \{ 0, 1\}^m$ uniformly at random.
	\item Let $i^\star = f(X_1, \ldots, X_m)$.
	\item Output bias vector $p = (\frac{1}{2} X_1, \ldots, \frac{1}{2} X_m) + e_{i^\star}$, where $+$ indicates appending vectors. 
\end{itemize}
For small enough $m$ relative to $K$, if $f$ is known, then a nearly-optimal strategy is to pull the information-revealing arms until we can distinguish between the case where the bias is 0 or $1/2$ for each, after which we pull the high-reward arm. The following lemma shows that this strategy yields high reward.

\begin{lemma}
\label{lem:approx-optimal-reward}
Pick $\delta > 0$ and prior $\mu_f$. There is a policy that achieves expected reward $(1-\delta)(H - m \log_2\frac{m}{\delta})$.
\end{lemma}
\begin{proof}
Let $f : \{0,1 \}^m \rightarrow [K]$ be the underlying function. For each information revealing arm $i$, pull it $\log_2	\frac{m}{\delta}$ times. If any of the pulls comes up 1, set $\hat{x}_i = 1$, otherwise set $\hat{x}_i = 0$. For the rest of the rounds, pull arm $f(\hat{x})$. Let $X = (X_1, \ldots, X_m)$ be the true values of the information revealing arms. We have with probability at least $1-\delta$ that $\hat{x} = X$. Conditioned on this occurring, the reward in this round will be at least $H - m\log_2	\frac{m}{\delta}$. Taking expectations gives us the lemma.
\end{proof}

As a consequence of Lemma~\ref{lem:approx-optimal-reward}, one can show that any policy that does not choose the optimal arm within a small number of pulls must suffer large expected regret.

\begin{lemma}
\label{lem:reward-lower-bound}
Pick a prior $\mu_f$ and fix a policy with expected regret less than $H/64$ (measured against the optimal policy). Then in each meta-round, with probability at least 1/2, the policy must choose the optimal arm within the first ${H}/{8} + \frac{63}{16} m \log_2(64 m)$ pulls.
\end{lemma}
\begin{proof}
Suppose by contradiction that with probability at least 1/2, the policy does not choose the optimal arm within the first ${H}/{16} + m \log_2(64 m)$ rounds. As the maximum expected reward of any non-optimal arm is 1/2, the expected reward of this policy is at most
\[ \frac{1}{2} H + \frac{1}{2} \left(H - \frac{1}{2}\left(\frac{1}{8}H + \frac{63}{16} m \log_2(64 m) \right) \right) \ = \ \frac{31}{32} H - \frac{63}{64} m \log_2(64 m)). \]
On the other hand, Lemma~\ref{lem:approx-optimal-reward} with $\delta = 1/64$ says that there is a policy with expected reward at least 
\[ \frac{63}{64} (H - m \log_2(64 m)). \] 
Taking differences, we see a difference of at least $H/64$, providing us with a contradiction.
\end{proof}

Thus, we can think of a low-regret learner as a function $\pi: \{ 0, 1 \}^m \rightarrow {[K] \choose r}$ where we have the true arm in $\pi(x)$ with reasonably large probability. The following No Free Lunch-style theorem shows that with constant probability, any learning algorithm that outputs such a function must suffer large regret whenever the number of training examples is not large enough.

\begin{theorem}[No free lunch for set prediction]
\label{thm:nflt}
Let $\X$ be a finite data space, $K \geq 2$, and say $n < |\X|$ and $r < K$. Let $A$ be any algorithm that takes as input a sequence of examples $S = ((x_1, y_1), \ldots, (x_n, y_n)) \in (\X \times [K])^n$ and outputs a set predictor $A(S): \X \rightarrow {[K] \choose r}$. Then there exists a function $f:\X \rightarrow [K]$ such that the distribution $\D_f$ given by 
\[ \D_f((x,y)) \ = \ \begin{cases}
1/|\X| & \text{ if } y = f(x) \\
0 & \text{ else}
\end{cases} \]
satisfies that $\E_{S \sim \D_f^n}[L_{\D}(A(S))]  \geq  \frac{|\X| - n}{|\X|} \cdot \frac{K-r}{K}$, where $L_{\D_f}(\pi) := \pr_{(x,y) \sim \D}(y \not \in \pi(x))$. As a consequence, with probability at least 1/4 over the draw of $S \sim \D_f^n$, we have $L_{\D_f}(A(S)) \geq \frac{1}{3}\left(\frac{4(|\X| - n)(K-r)}{|\X| K} - 1\right)$.
Moreover, this holds even if $A$ is a randomized algorithm that produces a randomized set predictor.
\end{theorem}
\begin{proof}
The proof is an adaptation of the one given for Theorem 5.1 in~\cite{SB14}.

Let $f_1, \ldots, f_T$ denote all possible $K^{|\X|}$ functions from $\X$ to $[K]$. For any $t \in [T]$, let $\D_t$ denote the distribution
\[ \D_t((x,y)) \ = \ \begin{cases}
1/|\X| & \text{ if } y = f_t(x) \\
0 & \text{ else}.
\end{cases} \]
We will show that for any algorithm $A$ that receives a training set $S$ of $n$ examples, it holds that
\[ \max_{t \in [T]} \E_{S \sim \D_t^n}[L_{\D_t}(A(S))] \ \geq \ \frac{|\X| - n}{|\X|} \cdot \frac{K-r}{K} .\]
Note that the number of possible length $n$ sequences from $\X$ is $N:= |\X|^n$. Call these sequences $S_1, \ldots, S_N$. For any sequence $S_j = (x_1, \ldots, x_n)$, let $S^{(t)}_j = ((x_1, f_t(x_1)), \ldots, (x_n, f_t(x_n)))$. Then $\D_t^n$ is uniform over $S^{(t)}_1, \ldots, S^{(t)}_N$. Thus,
\begin{align*}
\max_{t \in [T]} \E_{S \sim \D_t^n}[L_{\D_t}(A(S))] \ &= \ \max_{t \in [T]} \frac{1}{N} \sum_{j=1}^N L_{\D_t}(A(S^{(t)}_j)) \\
\ &\geq \ \frac{1}{T} \sum_{t=1}^T \frac{1}{N} \sum_{j=1}^N L_{\D_t}(A(S^{(t)}_j)) \\
\ &= \ \frac{1}{N} \sum_{j=1}^N \frac{1}{T} \sum_{t=1}^T  L_{\D_t}(A(S^{(t)}_j)) \\ 
\ &\geq \ \min_{j \in [N]} \frac{1}{T} \sum_{t=1}^T  L_{\D_t}(A(S^{(t)}_j)).
\end{align*}
Now pick any $j \in [N]$. Let $S_j = (x_1, \ldots, x_n)$ and let $z_1, \ldots, z_p$ be the elements of $\X$ that do not appear in $S_j$. Note that $p\geq |\X| - n$. Then for every 
$\pi: \X \rightarrow {[K] \choose r}$,
\begin{align*}
L_{\D_t}(\pi) \ &= \ \frac{1}{|\X|} \sum_{x \in \X} \ind[f_t(x) \not \in \pi(x)] \\
\ &\geq \ \frac{1}{|\X|} \sum_{i=1}^p \ind[f_t(z_i) \not \in \pi(z_i)] \\
\ &= \ \frac{p}{|\X|} \cdot \frac{1}{p} \sum_{i=1}^p \ind[f_t(z_i) \not \in \pi(z_i)].
\end{align*}
Thus,
\begin{align*}
\frac{1}{T} \sum_{t=1}^T  L_{\D_t}(A(S^{(t)}_j)) \ &\geq \ \frac{p}{|\X|} \cdot \frac{1}{T} \sum_{t=1}^T  \frac{1}{p} \sum_{i=1}^p \ind[f_t(z_i) \not \in A(S^{(t)}_j)(z_i)] \\
\ &= \ \frac{p}{|\X|} \cdot \frac{1}{p} \sum_{i=1}^p \frac{1}{T} \sum_{t=1}^T \ind[f_t(z_i) \not \in A(S^{(t)}_j)(z_i)] \\
\ &\geq \ \frac{|\X| - n}{|\X|} \min_{i \in [p]} \frac{1}{T} \sum_{t=1}^T \ind[f_t(z_i) \not \in A(S^{(t)}_j)(z_i)].
\end{align*}
Now fix any $i \in [p]$. We may partition the functions $f_1, \ldots, f_T$ into $T/K$ disjoint $K$-tuples of the form $(f_{t_1}, \ldots, f_{t_K})$ such that for every tuple and every $x \in \X$, we have
\begin{align*}
|\{ f_{t_1}(x), \ldots, f_{t_K}(x)\}| \ = \ \begin{cases}
K &\text{ if } x = z_i \\
1 & \text{ else}.
\end{cases}
\end{align*}
Note that this implies $S_j^{(t_1)} = S_j^{(t_2)} = \cdots = S_j^{(t_K)}$. Thus,
\[ \sum_{k=1}^K \ind\left[ f_{t_k}(z_i) \in A(S_j^{(t_k)}) \right] \ = \ K-r \]
and therefore
\[ \frac{1}{T} \sum_{t=1}^T  \ind[f_t(z_i) \not \in A(S^{(t)}_j)(z_i)] \ = \ \frac{K-r}{K}.  \]
Using our inequalities from above, we have
\[ \max_{t \in [T]} \E_{S \sim \D_t^n}[L_{\D_t}(A(S))] \ \geq \  \frac{|\X| - n}{|\X|} \cdot \frac{K-r}{K}. \]
To see that all of the above holds even for randomized algorithms over randomized set predictors, we separate out the internal randomness of $A$ into an independent random variable $b$ and the internal randomness of the predictor into an independent random variable $b'$, say in some space $\B$. Then the learning algorithm takes as input a training set $S$ and a random variable $b$ and outputs a function $A(S,b): \X \times \B \rightarrow {[K] \choose r}$. Then our goal can be rewritten as
\[ \max_{t \in [T]} \E_{S \sim \D_t^n, b, b'}[L_{\D_t}(A(S,b)[b'])] 
\ := \ \max_{t \in [T]} \E_{S \sim \D_t^n, b} \left[\pr_{(x,y)\sim \D_t, b'} \left( y \not \in A(S,b)[x,b'] \right)  \right]
\ \geq \ \frac{|\X| - n}{|\X|} \cdot \frac{K-r}{K} .\]
The proof of this follows the same steps as before, keeping careful track of the random variables $b$ and $b'$ and conditioning on them when appropriate.
\end{proof}

Putting it all together, we have the following.

\begin{theorem}
Suppose that $K > \frac{5}{3} \left( {H}/{8} + \frac{63}{16} m \log_2(64 m) \right)$, $H > \frac{63}{14}m \log_2(64 m)$, and $m > 5$. Fix any meta-learning algorithm $A$ and any number of meta-rounds $T \leq 2^{m-4}$. Then there is a prior distribution $\mu_f$ such that with probability at least $1/4$, the policy output by the meta-learning algorithm after $T$ meta-rounds will have expected regret at least $H/64$.
\end{theorem}
\begin{proof}
We will show that a low-regret meta-learning algorithm can be turned into a randomized set prediction algorithm in the style of Theorem~\ref{thm:nflt}. To begin, suppose $\D$ is a distribution over $\{0,1 \}^m \times [K]$ such that there exists a function $f: \{0,1 \}^m \rightarrow [K]$ where $\D((x,y)) > 0$ implies $y = f(x)$.


For any $(x, y) \sim \D$, define the bias vector $p = \frac{1}{2}x + e_y$. That is, the $i$-th information revealing arm has bias $x_i/2$ and the $j$-th potential reward arm is 1 if and only if $j = y$. Thus, $\D$ induces a prior distribution $\mu_f$ over bias vectors, and for any dataset $S \sim \D^T$, we may use $S$ to simulate $T$ draws from the prior $\mu_f$. Moreover, it is easy to see that we can run our meta-learning algorithm on these inputs, drawing rewards from the appropriate Bernoulli distributions and faithfully simulating $T$ meta-rounds of the prior $\mu_f$. 


At the end of these $T$ meta-rounds, the meta-learning algorithm will produce a policy. To convert this into a set predictor $\pi:  \{0,1 \}^m \rightarrow {[K] \choose r}$, on input $x \in \{ 0,1\}^m$ we will simulate the policy as follows:
\begin{itemize}
	\item If the policy pulls an information revealing arm $i$, we will draw its reward from Bernoulli$(1/2)$.
	\item If the policy pulls a potential reward arm, we will return the reward 0.
\end{itemize}
The prediction of the policy on $x$ is given by the first $r$ arms it pulls. Note that up until the policy pulls arm $f(x)$, this is a faithful simulation of the true environment. 

If our policy has expected regret less than $H/64$ with respect to $\mu_f$, then by Lemma~\ref{lem:reward-lower-bound} with probability at least 1/2 the policy must pull arm $f(x)$ in the first $r = {H}/{8} + \frac{63}{16} m \log_2(64 m)$ pulls. This implies that the randomized set predictor $\pi$ induced by our policy satisfies $L_{\D}(\pi) \leq 1/2$. 

On the other hand, Theorem~\ref{thm:nflt} tells us that for any (possibly randomized) learning algorithm must, there exists a distribution $\D$ such that with probability at least $1/4$ over the draw of the training set of size $T$, the randomized set predictor will have error at least 
\[ \frac{1}{3}\left(\frac{4(2^m - T)(K-r)}{2^m K} - 1\right) > \frac{1}{2} \]
where we have used the inequalities $T \leq 2^{m-4}$ and $K  >  \frac{5}{3} \left( {H}/{8} + \frac{63}{16} m \log_2(64 m) \right) = 5r/3$ from the theorem statement.

Thus, for any meta-learning algorithm, there exists a prior distribution $\mu_f$ such that with probability at least $1/4$, the policy produced by the meta-learning algorithm after $T \leq 2^{m-4}$ meta-rounds must have expected regret at least $H/64$.
\end{proof}

To fulfill the conditions of the theorem, we can take $m = cK/\log_2 K$ for some small enough constant $c > 0$. Then the total number of arms is $O(K)$, the horizon $H$ is $O(K)$, and the lower bound on the number of meta-rounds is $2^{ \Omega(K/\log_2 K)}$.

==> body/model.tex <==
%!TEX root = ../main.tex


\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\renewcommand{\E}{\mathbb{E}}


\section{Model}
A meta-prior $N(\vec\theta,\Sigma)$ and MAB instances $\vec{\mu}^t\sim N(\vec{\theta},\Sigma)$ are drawn for each meta-round $t=1,\ldots, T$. $\Sigma$ captures the correlations between means of the arms
For each base round $k=1,\ldots,K$, rewards for each is $r^{t,k}(a)\sim \mathcal{N}(\mu^t(a), 1)$. The noise is independent across arms (and of known variance). 

We assume that base learners employ posterior sampling (Algorithm in \cite{RussoRoyMOR14})  and the meta-learner selects their prior. If the meta-learner provides the correct prior then the base learner runs exactly the algorithm of Russo and van Roy \cite{RussoRoyMOR14} since the latter is Bayesian. 

However, by offering erroneous priors, the meta-learner can make the base learner act in ways that are more exploration-heavy (and can help meta-learn the underlying parameters of the meta-prior). For example, by imposing a $\Sigma$ that tells that all arms have the same (correlated) mean, the meta-learner can make the base-learner continuously exploring uniformly at random.

\subsection{Competing against ex-ante optimal arm}
Regardless of the base horizon $K$ (even for $K=1$), we can always achieve $K\sqrt{T}$ meta-regret against the ex ante optimal arm by applying any bandit algorithm, keep selecting this arm throughout the whole base learning algorithm and returning the average reward over its lifetime.

\subsection{Competing against ex-post optimal arm}
If the base horizon $K$ is large then we can use the initial $T^{2/3}$ rounds by uniformly exploring arms (as described above). At this point, we can estimate $\vec{\theta}$ and subsequently also estimate $\Sigma$ at a precision of $\epsilon=T^{-1/3}$. After this point, we can use the resulting prior. Since the algorithm of Russo and van Roy is approximation-preserving, we lose an additional $T^{2/3}$ in the remaining rounds.

\subsection{Open questions}
First, it would be great to move beyond $T^{2/3}$. Unfortunately, this is challenging as, with adaptive sampling, classical estimators are no longer unbiased and adaptive sampling is necessary for anything that does not separate exploration and exploitation.

Second, it would be interesting to think about how the guarantees depend on the base horizon. When $K=1$, we can really only hope for ex-ante guarantees. When $K$ is large, we can also get ex-post guarantees.

Third, for the covariance estimation, it is crucial that the noise variance is known (otherwise it is unclear what should be subtracted from the resulting distribution).

Fourth, we may want to explore guarantees as a function of the feedback received. 

Last, the base learner may be solving Bayesian best arm identification rather than regret.

\subsection{UCB+Thompson}
In each meta round $t$, the true mean is $\mu_t$. We get $\hat{\mu}_t$ and $\mathrm{ucb}_t$ such that
\begin{align*}
    \mu_t(a) \leq \hat{\mu}_t(a) + \mathrm{ucb}_t(a)
\end{align*}
After round $t$, we define
\begin{align*}
    \hat{\theta}_t = \frac{1}{t}\sum_{\tau=1}^t \hat{\mu}_\tau(a) + \mathrm{ucb}_\tau(a) + \sqrt{\frac{1}{t}}
\end{align*}
The $\sqrt{\frac{1}{t}}$ is to account for the fact that the average of the $\mu_\tau$'s itself would only be close to $\theta$. It should be pretty easy to prove that $\theta \leq \hat{\theta}_t$ pointwise. But it seems unlikely that $\hat{\theta}_t \leq \theta + o(T)$, so this would not work. 

Let's say we get $\hat{\mu}_t$ and $N_t$, the latter of which is the counts for each arm. Now, a pretty good estimate of $\theta$ should be
\begin{align*}
    \theta(a) \approx \frac{\sum_{t=1}^T {N_t(a)\hat{\mu}_t(a)}}{\sum_{t=1}^T N_t(a)}
\end{align*}
This one is less clear if it works. 


\subsection{Connection to Truncated Gaussians to deal with bias}


% \subsection{Russo-van Roy base learners}
% If the base horizon is large (to be defined) then two-stage process:
% \begin{itemize}
%     \item Uniformly explore actions (skewed prior) and use this to learn meta-prior (Give as prior any prior where all the arms have the same mean.)
%     \item Then use this meta-prior
%     \item This works for any $\Sigma$
% \end{itemize}
% \begin{theorem}
% For any $\Sigma$ (with bounded eigenvalues), if base horizon is large, this gives meta regret of $T^{2/3}$ (crucially needs knowledge of noise variance)
% \end{theorem}
% \begin{proof}{(sort of)}
% After $1/\epsilon^2$ exploration rounds, you identify an $\epsilon$-accurate prior (in these rounds, you uniformly select actions so you lose everything). After that, you lose $\epsilon\cdot T$. Setting $\epsilon=T^{-1/3}$, you get regret of $T^{2/3}$.
% \end{proof}

% Example: $\bar{r} \sim N(0, \sigma^2)$, $\epsilon \sim N(0, 1)$. We actually observe $\bar{r} + \epsilon$, and denote $y : = \bar{r} + \epsilon$. 

% We will get $\{ y_1, \dots, y_N \}$. We set mean as $\bar{y} = \sum_{i=1}^N y_i / N \to 0$. 

% But my empirical estimate of variance, which is $\frac{1}{N} \sum_{i=1}^N (y_i - \bar{y})^2 \to \sigma^2 + 1$, because $y \sim N(0, \sigma^2 + 1)$.

% \begin{remark} If noise variance is known then just decrease empirical variance by $1$ (noise variance). If it is unknown then this does not work
% \end{remark}

% \begin{itemize} 
% \item Vasilis' paper \end{itemize}

% \newpage

% \section{Model}
% The environment consists of a distribution across $N$ multi-armed bandit instances $\mathcal{M}=\{\mathcal{M}_i\}_{i=1}^N$, each of which appears with some measure $q_i$. All instances consists of $k$ arms. For simplicity, we assume that the set $\mathcal{M}$ is finite. The meta-learner knows the set of instances but does not know the corresponding measures. 

% The protocol for the base learner is the following. One instance $\mathcal{M}_i$ is drawn from the distribution. The base learner interacts $H$ times with the instance (these rounds do not count towards reward). In the end, the base learner selects an arm and earns the reward of the selected arm.

% The goal is to compare to the best adaptive query policy that queries arms. If $H$ really large then we can learn the best ex-post arm. If $H=0$, then we can only compete against the best ex-ante arm.

% Questions:
% \begin{itemize}
%     \item Power of static policies? How many rounds of adaptivity are needed?
%     \item Communication returned to the meta learner? Can returning only the final reward be useful?
%     \item Statistical benefits of meta learning?
% \end{itemize}

% \subsection{July 23}
% \begin{itemize}
%     \item Maybe Bayesian version of Sepehr's result on rounds of adaptivity
% \end{itemize}




% \newpage

% \section{Meeting of 3/12}
% \subsection{Protocol}
% There is a set of states $S$ and a set of actions $A$.

% There is a fixed external reward function $\rho(x,a,x')$; this is known to the meta-learner, crucially depends on the next state $x'$, in principle could also only depend on that.

% There is also a fixed distribution $\mathcal{D}$ over possible transition functions; this is unknown to the meta-learner. 

% Last, there is a policy class $\Pi:S\rightarrow A$ over which the base-learner's algorithm (say EXP4) optimizes over.

% For meta-round $t=1\ldots T$:
% \begin{enumerate}
%     \item Meta-learner chooses $R_t(x,a,x')$; this is the myopic reward (taken from some class $\textbf{R}$.
%     \item Nature chooses traansition function $P_t\sim\mathcal{D}$
%     \item The base learner runs $K$ episodes. For $k=1\ldots K$, itActs for $H$ steps by running EXP4 on $R_t$ (EXP4 observes context $x$, picks action $a$ and then observers the myopic reward $r=R_t(x,a,x')$.
%     \item The meta learner then observes the accrued external reward $\rho_t=\sum_{k=1}^K\sum_{h=1}^H \rho(x_{k;h},a_{k;h},x_{k;h+1})$ (or maybe the meta-learner observes the whole history). 
% \end{enumerate}
% The benchmark we compare against is $\max_{R\in\mathbf{R}} E[\rho(x,a,x')|EXP4 on R]$



% \subsection{Naive thought}
% \begin{itemize}
%     \item If there is only a finite set of $R$'s to choose from, the meta-learner just solves a bandit problem and the regret scales with the number of the policies. \akcomment{Reward functions, not policies!}
% \end{itemize}
% \subsection{Questions}
% \begin{itemize}
%     \item Can we get a better regret bound? (better than $poly(|\mathbf{R}|)$)
%     \item Compete with $\pi\in\Pi$ that optimizes $\max_\pi E_{\mathcal{D}}E_{\pi}[\rho(x,a,x')$
%     \item Are there natural settings where we can compute with $E_{\mathcal{D}}[\max_{\pi}E_{\pi}[\rho(x,a,x')]$
% \end{itemize}

% \subsection{Observations}
% \begin{itemize}
%     \item What about dependence on $H$?
%     \item For a given $R$ and $P$, EXP4 converges to a single deterministic policy.
% \end{itemize}

% \section{Pre-March version}
% We study a reinforcement learning setting with a state space $\states$ and an action space $\actions$. 

% A meta-learner has access to a policy space $\Pi$ and would like to perform well with respect to a deterministic \emph{extrinsic reward function} $r^{\star}:\states\times\actions \rightarrow \mathbb{R}$. The meta-learner can make changes every meta-step which we denote by $t=1,\ldots, T$. At the beginning of each meta-step, the learner commits to a (possibly randomized) \emph{intrinsic reward function} $R^{(t)}:\states\times \actions\rightarrow \mathbb{R}$.

% At each meta-step, a different base learner gets initialized and runs a contextual bandit algorithm; for instance EXP4 on the policy space $\Pi$ receiving as rewards the intrinsic rewards $R^{(t)}$ selected by the meta-learner. \tlcomment{possibly we could talk about losses and assume that the base learner runs make the minority great again so that we have a small-loss bound for the base learner.} 

% The base learner runs $M$ base-episodes which we refer to as $m=1,\ldots, M$. At the beginning of each base-episode, an initial state is selected at random. Each episode has $H$ base-steps which we refer to as $h=1,\ldots, H$. At every base-step, the contextual bandit algorithm (initialized in the beginning of the meta-step) observes a context $x_{t,m,h}$ associated to the current state $s_{t,m,h}$, selects an action $a_{t,m,h}$ and observes the intrinsic reward $R^{(t)}(s_{t,m,h},a_{t,m,h})$; then the distribution is updated based on these intrinsic rewards.. 

% \paragraph{Aftermaths from meeting of 2-21-2020.}
% \begin{enumerate}
%     \item Providing the extrinsic rewards as intrinsic is bad until at least $M=\Omega(2^H)$. \tlcomment{This is due to a combination lock example}
%     \item The optimal intrinsic reward depends on $M$ \tlcomment{$M=1$ and $M=\infty$ have different optimal intrinsic rewards in the same combination lock example}
%     \item If $M=poly(H)$ then giving intrinsic reward of $\mathbf{1}\{a=\pi^{\star}(x)\}$ where $
%     \pi^{\star}=\max_{\pi\in \Pi} V(\pi)$. \tlcomment{Wen
%     s conjecture}
% \end{enumerate}

% \paragraph{More than one MDPs.} 
% \begin{itemize}
%     \item know the identity of the MDP in the end
%     \item occupancy measure with different bonuses for the two
% \end{itemize}

% \section{March 12 version}

% There is a fixed external reward function $\rho \colon X \times A \times X \to \mathbb{R}$ (known to the metalearner), and a fixed distribution $D$ over possible transition functions (unknown to the metalearner).
% The base learner, who uses Exp4, is using a fixed policy class $\Pi \subseteq A^X$ comprised of policies $\pi \colon X \to A$.

% The protocol is as follows.
% \begin{itemize}
%   \item For meta-round $t=1,\dotsc,T$:
%     \begin{itemize}
%       \item Meta-learner chooses a ``myopic'' reward function $R_t \colon X \times A \times X \to \mathbb{R}$ from some class of reward functions $\mathcal{R}$.
%       \item Nature chooses a transition function $P_t \sim D$.
%       \item For episode $k=1,\dotsc,K$:
%         \begin{itemize}
%           \item An initial context $x_{k,1}$ is drawn from the starting state.
%           \item For step $h=1,\dotsc,H$:
%             \begin{itemize}
%               \item The base learner observes the context $x_{k,h} \in X$, chooses an action $a_{k,h} \in A$.
%               \item The state changes according to $P_t$, and the next context $x_{k,h+1}$ is drawn.
%               \item The base learner receives and observes the myopic reward $R_t(x_{k,h},a_{k,h},x_{k,h+1})$ (but the actual reward accrued is $\rho(x_{k,h},a_{k,h},x_{k,h+1})$).

%             \end{itemize}
%         \end{itemize}
%       \item The meta-learner observes the actual reward accrued by the base learner
%         \[
%           \rho_t := \sum_{k=1}^K \sum_{h=1}^H \rho(x_{k,h},a_{k,h},x_{k,h+1}) =: \widehat{\mathbb{E}}[ \rho(x,a,x') \mid \text{Exp4 on $R_t$} ] .
%         \]
%         (Or perhaps the meta-learner observes the whole history?)
%       \end{itemize}
% \end{itemize}

% A natural benchmark is
% \[
%   R^\star := \max_{R \in \mathcal{R}} \mathbb{E}[ \rho(x,a,x') \mid \text{Exp4 on $R$} ] .
% \]

% Naively: if $\mathcal{R}$ is finite, then the meta-learner ``just'' needs to solve a bandit problem (but regret could scale poorly, e.g., linearly in $|\mathcal{R}|$).

% Questions:
% \begin{enumerate}
%   \item Can we get a better regret bound? Better than $poly(|\mathcal{R}|)$?
%   \item Can we compete with
%     \[
%       \max_{\pi \in \Pi} \mathbb{E}_D \mathbb{E}_\pi[ \rho(x,a,x') ] ?
%     \]
%   \item Are there natural settings where it is possible to compete with
%     \[
%       \mathbb{E}_D\left[ \max_{\pi \in \Pi}  \mathbb{E}_\pi[ \rho(x,a,x') ] \right] ?
%     \]
%   \item (AK question) Why does $P_t \sim D$ need to be stochastic? I am wondering if we could just do the adversarial version where $P_t$ is chosen by an (adaptive) adversary on each meta-round and we compute with 
%   \begin{align*}
%       \textrm{Bench}(\mathcal{R}) := \max_{R \in \mathcal{R}} \sum_{t=1}^T \mathbb{E}[\rho(x,a,x') \mid \textrm{Exp4 on } R \textrm{ with dynamics } P_t]
%   \end{align*}
%   It seems strictly more general and perhaps not actually that different. 
% \end{enumerate}


% \newcommand{\pigrd}{\pi^{\mathrm{grd}}}
% \section{Notes}
% I feel we need a "structural" result about the following object. Let $\pigrd_{R,P}$ denote the greedy policy for reward function $R$ and dynamics $P$, that is $\pigrd_{R,P}(x) := \argmax_{a} \mathbb{E}[R(x,a,x') | x' \sim P(\cdot \mid x,a)]$. Note that $\pigrd_{R,P}$ really does depend on $P$ because $R$ depends on the realization of $x'$. I am thinking we should try to show two things
% \begin{itemize}
%     \item Extrinsic reward for Exp4 on $(R,P)$ converges to $V(\pigrd_{R,P} | \rho, P)$. This seems intuitive to me.
%     \item For any $P$, there is some structure to the map $R \mapsto V(\pigrd_{R,P} | \rho, P)$. An immediate observation here is that even for each $P$, even though the domain is infinite, the range has only finitely many values, since there are only $A^S$ policies that $\pigrd$ could take. 
% \end{itemize}

% \subsection{Representing $R$ generically}

% Consider the set $S(\mathcal{R})=\{ (V_{R,P,\rho})_{P}: R\in\mathcal{R}\}$.
% Can we pick a subset $\mathcal{R}'\subseteq\mathcal{R}$, such that $S(\mathcal{R}')$ covers $S(\mathcal{R})$ in $\ell_\infty$ norm?

% Instead of $\pi^\text{grd}_{R,P}$ we should consider something like:
% \[
%   \pi^{\lambda}_{R,P}\coloneqq
%   \argmax_{\pi:\text{distance}(\pi,\text{uniform})\le\lambda}
%   \E_s \E_{a\sim\pi(\cdot | s)} \E_{s'\sim P(\cdot\mid s,a)} [R(s,a,s')]
% \]
% This seems to require to specify some measure over $s$ with respect which
% to optimize.

% \section{Meeting of March 19}

% \paragraph{Simple observation}
% $r(x,a)=E_P[R(x,a,x') | x,a]$

% If $P(x'|x,a)\in\mathcal{P}$ of dim $d$ then $R$ can be chosen of dim $d$

% \subsection{LQR}
% LQR is specified by
% \begin{align*}
%     x_{t+1} = Ax_t + Bu_t + \epsilon_t \qquad c_t = x_t^\top Q x_t + u_t^\top R u_t
% \end{align*}
% where $(Q,R)$ are the cost functions. It is know that the optimal controller $\pi^\star$ is a linear map, which means that $\pi^\star(x) = K^\star x$ for all $x$, where $K^\star$ is a matrix given by solving the discrete Algebraic Ricatti Equation. Intuition: Value function (w.r.t., $Q^\star, R^\star$) of the optimal controller for $(Q,R)$ can be written in closed form (AK thinks). 

% Maybe here is a different LQR formulation:
% \begin{align}
%     x_{t+1} = Ax_t + Bu_t + \epsilon_t, \qquad c_t = x_{t+1}^\top Q x_{t+1} + u_t R u_t \label{eq:lqr_one_step}
% \end{align}
% \subsection{Another idea: can we leverage Karan's reduction?}

% \subsection{For MDP}
% For discounted MDP, for any policy $\pi$ (perhaps $\pigrd_{R,P}$). The bellman equation is that
% \begin{align*}
%     V = P^\pi (\rho + \gamma V)
% \end{align*}
% And so:
% \begin{align*}
%     V = (I - \gamma P^\pi)^{-1} P^\pi \rho
% \end{align*}

% \subsection{Questions}

% \begin{itemize}
% \item For LQR setting (e.g.,~\eqref{eq:lqr_one_step}: Can we verify:
% \begin{enumerate}
%     \item $\pigrd_{R,P}$ is a linear controller
%     \item $V(\pigrd_{R,P} | \rho, P)$ is quadratic in $x$. How does it depend on $R$?
% \end{enumerate}
% \end{itemize}


==> body/prelim.tex <==
%!TEX root = ../main.tex

\section{Towards a Problem Formulation}
\newcommand{\ahat}{\widehat{a}}
\newcommand{\prior}{\mathsf{P}_{\star}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\Alggold}{\Alg_{\mathrm{gold}}}
\newcommand{\Rew}{\mathrm{Rew}}
\newcommand{\ERew}{\mathbb{E}\text{-}\mathrm{Rew}}
\newcommand{\RewExpPost}{\mathrm{ExPost}}
\newcommand{\Reg}{\mathrm{Reg}}
\newcommand{\BigOh}[1]{\mathcal{O}(#1)}
\newcommand{\Alg}{\mathsf{alg}}

We consider an episodic multi-armed bandit problem with $K$ arms, episodes of horizon $H$, and $T$ episodes. 

The rewards of the arms are drawn as $\mu_t \in \R^K \sim \prior = \calN(\mu_{0},\Sigma_{0})$; we denotes its entries $\mu_{t,a} \in \R$. We assume that the rewards from each arm are Gaussian $X_{a,t,h} \sim \mathcal{N}(\mu_{t,a},1)$. At the end of each episode $t$, the learner makes a recommendation $\ahat_t \in [K]$, on which the agent is evaluated. 

\paragraph{Comparator: } Let us now consider the comparator for this problem. We define the reward of our algorithm as
\begin{align*}
    \Rew_T(\Alg) := \sum_{t=1}^T \mu_{t,\ahat_t}.
\end{align*}
as the cumulative mean reward of the recommendation. For comparators, we consider a \emph{gold standard} algorithm $\Alggold$, which takes  as input, and consider its expected reward
\begin{align*}
    \ERew_T(\Alggold) = \sum_{t=1}^T \E[\mu_{t,\ahat_t} \mid \Alggold(\prior), \mu_{t}]
\end{align*}
as the sum of over the expected rewards of $\Alggold$, conditioned on the realizations $\mu_t$.
We may then consider
\begin{align*}
    \Reg_{T}(\Alg;\Alggold) := \Rew_T(\Alg) - \ERew_T(\Alggold). 
\end{align*}
The above may be also selected with simple regret.

\section{Approaches}

\begin{quote}
    What is the sensitivity of Thompson sampling to a mispecified prior?
\end{quote}
Potentially, if the sampling algorithm is consistent or "stable" in some way, then there is some to do this. 


\begin{itemize}
    \item Explore for $T^{2/3}$ steps, exploit the learned prior for the remainder. If TS is sufficiently robust to mispecification of the prior, this should be $T^{2/3}$-regret
    \item Suppose TS is guaranteed to supply some exploration, although biased. Can we use MAP to attain $\sqrt{T}$ regret?
    \item Is there ``directed exploration'' based on something like optimism to enjoy faster rates?
    \item lower bound to rule out $\log T$ regret. 
\end{itemize}



\section{Algorithms}
\newcommand{\Phat}{\widehat{\mathsf{P}}}
\subsection{Naive Algorithm: Explore Exploit}
Consider the following algorithm:
\begin{enumerate}
    \item Explore uniformly for $T_0 = T^{2/3}$ steps, and form an estimate $\Phat$. 
    \item Play $\Alggold(\Phat)$ for all $t \ge T$.
\end{enumerate}
\newcommand{\TV}{\mathrm{TV}}
To analyze this, we make the following observation
\begin{lemma} $\|\Phat - \prior\|_{\TV} \le \BigOh{1/\sqrt{T_0}}$
\end{lemma}
\begin{lemma} Suppose that $\|\Phat - \prior\|_{\TV} \le \epsilon \le 1/4$. Then, 
\begin{align*}
    \left|\E_{\mu \sim \prior} \left[\E[\mu_{\ahat} \mid \Alggold(\prior), \mu] - \E[\mu_{\ahat} \mid \Alggold(\Phat), \mu] \right]\right| \le \BigOh{\epsilon}.
\end{align*}
\end{lemma}




\newpage
\section{Gaussian Case}
\newcommand{\posterior}{P}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\dP}{\mathrm{d}\mathrm{Pr}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetach}{\check{\theta}}
\newcommand{\muhat}{\widehat{\mu}}
\newcommand{\mustar}{\mu^{\star}}
\newcommand{\Sigmastar}{\Sigma^{\star}}

\newcommand{\Sigmahat}{\widehat{\Sigma}}

Let $\mu_k \sim \calN(\mu^\star,\Sigma^\star)$. You want ``sufficient exploration`` in $\E_{\mu}[\text{Thompson Sampling}]$

At each round, I have a posterior $(\muhat_k, \Sigmahat_k) \sim P_k$, and then I assume that $\theta \sim \calN(\muhat_k,\Sigmahat_k)$. 
\newcommand{\data}{\mathsf{data}}
\begin{align*}
   \log  \dP_k(\mu,\Sigma) = C(\data_{1:k-1}) + \sum_{j=1}^{k-1} \log \dP  [\data_j \mid \mu,\Sigma] + \log \dP(\mu,\Sigma)
\end{align*}
\begin{itemize}
    \item Option 1: Use MAP/MLE to find $\mu_k,\Sigma_k$
    \item Option 2: Set $(\mu_k,\Sigma_k)$ via posterior.  
\end{itemize}
So what happens is
\begin{align}
     (\mu,\Sigma) &\in \argmax \sum_{j=1}^{k-1} \log \dP  [\data_j \mid \mu,\Sigma]\\
     &\in \argmax \sum_{j=1}^{k-1} \|\vec{T}_j\mubar_{j}  - \mu\|_{\Sigma}^2 - \log \det |\Sigma| 
\end{align}


\begin{assumption} Let $\mathcal{B} := \{(\mu,\Sigma) : \|\mu - \mustar\| + \|\Sigma - \Sigma_\star\| \le \dots\}$. Then, if I run TS with prior  $ p = \calN(\mu,\Sigma)$, and the ground truth is $(\mu_{\star},\Sigmastar)$, then I have
\begin{align*}
   \E_{\mu \sim \calN(\mu_{\star},\Sigmastar)} \E_{p \gets \calN(\mu,\Sigma)}[\|\vec{T}_j\mubar_{j}  - \mu\|_{\Sigma}^2 - \log \det |\Sigma|] \ge (\dots). 
\end{align*}
\end{assumption}

\begin{itemize}
    \item $T^{2/3}$ regardless
    \item If sufficient exploration, $\sqrt{T}$
    \item Maybe: aggressive exploration to go between the two
    \item Possibly: use optimism to get $\sqrt{T}$ regardless
\end{itemize}

\begin{comment}
\subsection{Greedy Exploration}
We have 



\section{Old} 
Finally, we define the \emph{ex-post} optimal reward as
\begin{align*}
    \RewExpPost := \sum_{t=1}^T \max_{a \in [K]} \mu_{t,a}.
\end{align*}
Our notion of performance is as follows:
\begin{align*}
    \Reg_{T,\alpha}(\Alg;\Alggold) := \Rew_T(\Alg) - \ERew_T(\Alggold) - \alpha (\RewExpPost -  \ERew_T(\Alggold) )
\end{align*}
In other words, how much worse does $\Rew_T(\Alg)$ perform relative to $\ERew_T(\Alggold)$, plus an additive multiplicative factor penalizing the suboptimality of $\Alggold$ relative to the expost optimal. 

For examle, $\Alggold$ is top-two sampling with the true prior. 
I believe we should be able to obtain the above with $\alpha = 0$. 

\end{comment}

==> body/smoothness.tex <==
%!TEX root = ../main.tex


\section{Sensitivity}
We consider a family of $n$-Monte Carlo Bayesian algorithms. Such algorithms have the following shape. There exists functions $f_1,f_2,\dots :\R^{n \times K} \to [K]$. Let $\traj_t =(a_1,r_1,\dotsc,a_t,r_t)$ denote trajectories of actions and rewards, and let $\Plawof{\theta}$ denote the distribution over trajectories where rewards are drawn from $\mustar$ with $\mustar \sim \prior(\theta)$. Then at times $t$, $\alg(\theta)$ draws 
\begin{align}
\muhat_{t,1},\dots \muhat_{t,n} \iidsim \Plawof{\theta}(\mustar \in \cdot \mid \traj_t),
\end{align}
and selects\mscomment{formalize that the posteriors don't depend on algorithm}
\mdcomment{maybe we can just change $\mustar$ to $\mu$ and treat
it as a random variable under $\theta$?}
\begin{align}
a_t = f_t(\muhat_{t,1},\dots \muhat_{t,n}).
\end{align}\dhcomment{Is there an off-by-one here? Since $\traj_t$ already contains $a_t$.}
This gives rise to laws over trajectories $\traj_t$ of the form $\Plawof{\theta}_{\alg(\theta')}$, that is, the laws of running $\alg(\theta')$ under the ground truth $\theta$. 

\begin{theorem} Let $\alg$ denote an $n$-Monte Carlo Bayesian algorithm. Then, for any $H$.
\begin{align}
\TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)} \le (2+4n)H \cdot \TV(\prior(\theta),\prior(\theta'))
\end{align}
\akcomment{I think should be $2n+4$?}\dhcomment{agreed, per the proof.}
\mdcomment{for consistency, we could write $\Plawof{\theta}(\mu)$ instead of $\prior(\theta)$}
\end{theorem}
\begin{proof} Let $\theta_1,\theta_2$ denote the two alternative instances. Let us denote $\Plawof{i}_{\alg(j)} = \Plaw^{\theta_i}_{\alg(\theta_j)}$ denote law of running $\alg(\theta_j)$ with rewards from $\mustar \sim \theta_i$. Furthermore, let $\signal_t = (a_1,r_1,\dotsc,a_{t-1},r_{t-1},a_t) $ denote the history at time $t$, omitting the last reward. Note that the conditional distribution of the trajectory $\traj_t$ \akedit{(which contains $r_t$)} given $\signal_t$ \akedit{(which does not contain $r_t$)} is determined by the conditional distribution of $r_t \mid a_t$, which is the same  for $\Plawof{i}_{\alg(1)}$ and $\Plawof{i}_{\alg(2)}$. Hence, $\TVof{\Plawof{1}_{\alg(1)}(\traj_H),\Plawof{1}_{\alg(2)}(\traj_H)}  = \TVof{\Plawof{1}_{\alg(1)}(\signal_H),\Plawof{1}_{\alg(2)}(\signal_H)}$, so it suffices to show
 \begin{align}
\TVof{\Plawof{1}_{\alg(1)}(\signal_H),\Plawof{1}_{\alg(2)}(\signal_H)} \le (2+4n)H \cdot \TVof{\prior(\theta_1),\prior(\theta_2)}. 
\end{align}
To bound the left-hand side, we introduce the following measures $\Plawof{i}_{t}$, which corresponds to the law of running $\alg(\theta_1)$ for $t$-steps, then switching to $\alg(\theta_2)$, under rewards drawn from $\mustar \sim \pi(\theta_i)$. 
\begin{lemma}[Performance Difference]\label{lem:perf_diff_one}
\begin{align}
\TVof{\Plawof{1}_{\alg(1)}(\signal_H),\Plawof{1}_{\alg(2)}(\signal_H)}\le \sum_{t=0}^{H-1}\TVof{\Plawof{1}_{\alg(1)}(\signal_{t+1}),\Plawof{1}_{t}(\signal_{t+1})}
\end{align}
\end{lemma}
This is a direct consequence of the following lemma, proven below:
\begin{lemma}[Performance Difference]\label{lem:perf_diff_general} Let $\Qlaw$ and $\Plaw$ be laws over a sequence $\matx_{1:H}$. For $t \in [H]$, define the swapped laws $\Qlaw_{t}(\matx_{1:t+1})$ where $\matx_{1:t} \sim \Plaw(\matx_{1:t})$ and $\matx_{t+1} \mid \matx_{1:t} \sim \Qlaw(\matx_{t+1} \in \cdot \mid \matx_{1:t})$. Then,
\begin{align*}
\TVof{\Plaw(\matx_{1:H}),\Qlaw(\matx_{1:H})} = %\TVof{\Plaw^{[0]}(\matx_{1:H}),\Plaw^{[H+1]}(\matx_{1:H})} \le 
\sum_{t=0}^{H-1} \TV(\Plaw(\matx_{1:t+1}),\Qlaw_{t}(\matx_{1:t+1}))
\end{align*}
\end{lemma}
Starting from \Cref{lem:perf_diff_one},
\begin{equation}
\label{eq:TV_decomp_thing}
\begin{aligned}
\TVof{\Plawof{1}_{\alg(1)}(\signal_H),\Plawof{1}_{\alg(2)}(\signal_H)}&\le \sum_{t=0}^{H-1}\TVof{\Plawof{1}_{\alg(1)}(\signal_{t+1}),\Plawof{1}_{t}(\signal_{t+1})}\\ %\tag{\Cref{lem:perf_diff_one}}
&\le \sum_{t=0}^{H-1}\TVof{\Plawof{1}_{\alg(1)}(\signal_{t+1}),\Plawof{2}_{t}(\signal_{t+1})} + \TVof{\Plawof{1}_{t}(\signal_{t+1}),\Plawof{2}_{t}(\signal_{t+1})}\\
&\le H\TVof{\pi(\theta_1),\pi(\theta_2)} + \sum_{t=0}^{H-1}\TVof{\Plawof{1}_{\alg(1)}(\signal_{t+1}),\Plawof{2}_{t}(\signal_{t+1})}.
\end{aligned}
\end{equation}
\akedit{The first inequality is~\Cref{lem:perf_diff_one}, the second is the triangle inequality, and third follows since the conditional distribution $\signal_{t+1} \mid \mustar$ is the same under $\Plawof{2}_{t}$ and $\Plawof{1}_{t}$. The latter holds since the algorithm is the same under the two measures.}
Let's introduce the shorthand $\muhat_{t;1:n} = (\muhat_{t,1},\muhat_{t,2},\dots,\muhat_{t,n})$
We now introduce the following claim
\begin{claim} The joint distributions of $W_{t} := (\mustar,\muhat_{t;1:n},\traj_t)$ under $\Plawof{1}_{\alg(1)}$ and $\Plawof{2}_{t}$ have the following properties:
\begin{itemize}
    \item $\Plawof{1}_{\alg(1)}[\traj_t \in \cdot \mid \mustar] = \Plawof{2}_{t}[\traj_t \in \cdot \mid \mustar]$\\
    \item Under both $\Plawof{1}_{\alg(1)}$ and $\Plawof{2}_t$,  $(\mustar,\muhat_{t,1},\muhat_{t,2},\dots,\muhat_{t,n})$ are independent and identically distributed given $\traj_t$. 
    \dhcomment{why does $\mustar$ have same conditional distribution as $\muhat_{t,1}$ given $\traj_t$ under $\Plawof{2}_t$? I believe it under $\Plawof{1}_{\alg(1)}$. But under $\Plawof{2}_t$, I thought we sample $\muhat_{t,1} \sim \Plawof{1}(\mustar \mid \traj_t)$. Maybe this is related to an off-by-one error, and really we should be talking about $\muhat_{t+1,1}$, which is sampled from $\Plawof{2}(\mustar \mid \traj_t)$.}
\end{itemize}
\end{claim}
Observe moreover that $\signal_{t+1}$ is a deterministic function of $W_t$ \akedit{(in particular it is the same function under $\Plawof{2}_{t}$ and $\Plawof{1}_{\alg(1)}$)}, and hence $\TVof{\Plawof{1}_{\alg(1)}(\signal_{t+1}),\Plawof{2}_{t}(\signal_{t+1})} \le \TVof{\Plawof{1}_{\alg(1)}(W_t),\Plawof{2}_{t}(W_t)}$. The following lemma controls this total variation:
\begin{lemma}\label{lem:info_thingy} Let $\Plaw$ and $\Qlaw$ denote two joint distributions  over random variables $(\mustar,\muhat_{1:n},\traj)$ where we adopt the shorthand  $\muhat_{1:n} = (\muhat_1,\dots,\muhat_n)$. Suppose that $\Plaw[\traj \in \cdot \mid \mustar] = \Qlaw[\traj \in \cdot \mid \mustar]$, and that $(\mustar,\muhat_{1:n})$ are i.i.d given $\traj$ under $\Plaw$ and $\Qlaw$.  Then, 
\begin{align*}
\TVof{\Plaw(W_t),\Qlaw(W_t)}  \le (2n + 3)\TVof{\Plaw(\mustar),\Qlaw(\mustar)}.
\end{align*}
\end{lemma}

Applying \Cref{lem:info_thingy}, 
\begin{align*}
\TVof{\Plawof{1}_{\alg(1)}(\signal_{t+1}),\Plawof{2}_{t}(\signal_{t+1})}  &\le \TVof{\Plawof{1}_{\alg(1)}(W_t),\Plawof{2}_{t}(W_t)} \\
&\le (2n+3)\TVof{\Plawof{1}_{\alg(1)}(\mustar),\Plawof{2}_{t}(\mustar)} = (2n+3)\TVof{\pi(\theta_1),\pi(\theta_2)}.
\end{align*}
The bound follows from \Cref{eq:TV_decomp_thing}.
\end{proof}

\subsection{Proof}
\begin{proof}[Proof of \Cref{lem:perf_diff_general}]
\mscomment{proof is terse. feel free to expound}
Define the augmented sequences $\matxbar_t = \matx_{1:t}$. Then, under the laws $\Plaw$ and $\Qlaw$, $\matxbar_t$ form a time inhomogenous Markov chain. It suffices to show 
 \begin{align*}
\TVof{\Plaw(\matxbar_{H}),\Qlaw(\matxbar_{H})} \akedit{\leq} %\TVof{\Plaw^{[0]}(\matx_{1:H}),\Plaw^{[H+1]}(\matx_{1:H})} \le 
\sum_{t=0}^{H-1} \TV(\Plaw(\matxbar_{t+1}),\Qlaw_{t}(\matxbar_{t+1}))
\end{align*}
Using the variation characterize of $\TV$, we have
\begin{align*}
\TVof{\Plaw(\matxbar_{H}),\Qlaw(\matxbar_{H})} = \sup_{\text{measurable } \calA \subset \calX_T} \Plaw[\matxbar_{H} \in \calA] - \Qlaw[\matxbar_{H} \in \calA].
\end{align*}
Fix any measurable $\calA$. Then, $\Plaw[\matxbar_{H} \in \calA]$ and $\Qlaw[\matxbar_{H} \in \calA]$ can be regarded as the expected reward under a Markov Reward process \mscomment{fill in details}, with $0$ reward for steps $t= 1,2,\dots,H-1$ and reward $\I\{\matxbar_H \in \calA\}$ at time $H$. By the performance difference lemma,
\begin{align*}
\Plaw[\matxbar_{H} \in \calA] - \Qlaw[\matxbar_{H} \in \calA] &= \sum_{t=0}^{H-1} \E_{\matxbar_t \sim \Plaw} (\Plaw[\cdot\mid \matxbar_{t}] - \Qlaw[\cdot \mid \matxbar_t]) [V^{\Qlaw}_{t+1}(\cdot )],
\end{align*}
where $V^{\Qlaw}_{t+1}(\cdot)$ is the value function of the MRP under $\Qlaw$. 
Since this value is at most one, $\E_{\matxbar_t \sim \Plaw} (\Plaw[\cdot\mid \matxbar_{t}] - \Qlaw[\cdot \mid \matxbar_t]) [V^{\Qlaw}_{t+1}(\cdot )] \le \E_{\matxbar_t \sim \Plaw}\TVof{\Plaw[\cdot\mid \matxbar_{t}],\Qlaw[\cdot \mid \matxbar_t])}$, which is precisely $\TVof{\Plaw(\matxbar_{t+1}),\Qlaw_t(\matxbar_{t+1})}$, as needed.
\end{proof}

\begin{proof}[Proof of \Cref{lem:info_thingy}]
\newcommand{\Plawtil}{\tilde{\Plaw}}
 Introduce the interpolating law $\Plawtil$, where $\Plawtil[\traj \in \cdot] = \Plaw[\traj \in \cdot]$, but $\Plawtil[(\mustar,\muhat_{1:n}) \in \cdot \mid \traj] = \Qlaw[(\mustar,\muhat_{1:n}) \in \cdot \mid \traj]$. By the triangle inequality,
\begin{align*}
\TVof{\Plaw(W_t),\Qlaw(W_t)} \le \TVof{\Plaw(W_t),\Plawtil(W_t)} + \TVof{\Plawtil(W_t),\Qlaw(W_t)}. 
\end{align*}
Since $\Plawtil[(\mustar,\muhat_{1:n}) \in \cdot \mid \traj] = \Qlaw[(\mustar,\muhat_{1:n}) \in \cdot \mid \traj]$, we have 
\begin{align}
\TVof{\Plawtil(W_t),\Qlaw(W_t)} = \TVof{\Plawtil(\traj),\Qlaw(\traj)} = \TVof{\Plaw(\traj),\Qlaw(\traj)}  \le \TVof{\Plaw(\mustar,\traj),\Qlaw(\mustar,\traj)}  \label{eq:PtilQ_bound}
\end{align}
On the other hand, since $\Plawtil[\traj \in \cdot] = \Plaw[\traj \in \cdot]$,
\begin{align*}
 \TVof{\Plaw(W_t),\Plawtil(W_t)} &= \E_{\traj \sim \Plaw} \TVof{\Plaw[ (\mustar,\muhat_{1:n}) \in \cdot \mid \traj], \Plawtil[ (\mustar,\muhat_{1:n}) \in \cdot \mid \traj]}\\
 &\overset{(i)}{\le} (n+1)\E_{\traj \sim \Plaw} \TVof{\Plaw[ \mustar \in \cdot \mid \traj], \Plawtil[ \mustar \in \cdot \mid \traj]}\\
 &=  (n+1)\TVof{\Plaw(\mustar,\traj),\Plawtil(\mustar,\traj)},
\end{align*}
where $(i)$ uses that $\Plawtil[ (\mustar,\muhat_{1:n}) \in \cdot \mid \traj] = \Qlaw[ (\mustar,\muhat_{1:n}) \in \cdot \mid \traj]$, and that under both $\Plaw$ and $\Qlaw$, $(\mustar,\muhat_{1:n})$ are a sequence of $n+1$ i.i.d. variables given $\traj$. Continuing, 
\begin{align*}
\TVof{\Plaw(\mustar,\traj),\Plawtil(\mustar,\traj)} \le \TVof{\Plaw(\mustar,\traj),\Qlaw(\mustar,\traj)} +\TVof{\Plawtil(\mustar,\traj),\Qlaw(\mustar,\traj)}.
\end{align*}
By data processing, $\TVof{\Plawtil(\mustar,\traj),\Qlaw(\mustar,\traj)} \le \TVof{\Plawtil(W_t),\Qlaw(W_t)}$, which we have already bounded by $\TVof{\Plaw(\mustar,\traj),\Qlaw(\mustar,\traj)}$ in \Cref{eq:PtilQ_bound}. Therefore, collecting our bounds thus far,
\begin{align}
\TVof{\Plaw(W_t),\Qlaw(W_t)} \le (1 + 2(n+1))\TVof{\Plaw(\mustar,\traj),\Qlaw(\mustar,\traj)} = (2n + 3)\TVof{\Plaw(\mustar,\traj),\Qlaw(\mustar,\traj)}.
\end{align}
Finally, since $\traj \mid \mustar$ is identically distributed under $\Plaw$ and $\Qlaw$, $\TVof{\Plaw(\mustar,\traj),\Qlaw(\mustar,\traj)} = \TVof{\Plaw(\mustar),\Qlaw(\mustar)}$.
\end{proof}

\subsection{A generalization}
\mscomment{ignore this for now sec for now}
The above does not apply to non-Monte Carlo algorithms. We can extend to algorithms that are not Monte Carlo, but are Monte Carlo-like. Given an increasing and concave function $\Psi: \R_+ \to \R_+$, we say a parametrized family of algorithms is $\Psi$ Bayesian if
\begin{align*}
\TVof{\Plaw_{\alg(\theta)}(a_t = \cdot \mid \traj_{t-1}), \Plaw_{\alg(\theta')}(a_t = \cdot \mid \traj_{t-1})} \le \Psi(\TVof{\Plawof{\theta}[\mustar \in \cdot \mid \traj_{t-1}), \Plawof{\theta'}[\mustar \in \cdot \mid \traj_{t-1}]} 
\end{align*}
For example: Thompson sampling satisfies the assumption with $\Psi(z) = z$ being the identity \akedit{by data-processing inequality}, Top-Two satisfies with $\Psi(z) = 2z$, $n$-monte carlo satisfies with $\Psi(z) = n\cdot z$, and maybe soft-max on conditional expectations holds for $\Psi(z) \sim \log z$?
\ctcomment{Pinsker's inequality can give us $\Psi(z) \leq \sqrt{2 \beta z}$ for soft-max on conditional expectations, where $\beta$ is the `temperature' parameter.}
\begin{theorem} Let $\Psi$ be increasing and concave, and let $\alg(\cdot)$ be a family of $\Psi$-Bayesian algorithms over parameters $\theta \in \Theta$. Then, for all $\theta,\theta' \in \Theta$,
\begin{align*}
\TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)} \le H\Psi\left(2\TVof{\prior(\theta),\prior(\theta')}\right).
\end{align*}
In particular, for Thompson Sampling,
\begin{align*}
\TVof{\Plawof{\theta}_{\TS(\theta)}(\traj_H),\Plawof{\theta}_{\TS(\theta')}(\traj_H)} \le 2H\TVof{\prior(\theta),\prior(\theta')}
\end{align*}
\end{theorem}



Note that $\Plawof{\theta}[\mustar \in \cdot \mid \traj_{t-1}]$ is independent of the algorithm used to collect $\traj_{t-1}$. Using performance difference followed by Jensen's
\begin{align*}
\TVof{\Plawof{1}_{\alg(1)}(\traj_H),\Plawof{1}_{\alg(2)}(\traj_H)}&\le \sum_{t=0}^{H-1}\Expop_{\traj_t \sim \Plawof{1}_{\alg(1)}}\TVof{\Plaw_{\alg(1)}(a_t = \cdot \mid \traj_{t}),\Plaw_{\alg(2)}(a_t = \cdot \mid \traj_{t})}\\
&\le \sum_{t=0}^{H-1}\Expop_{\traj_t \sim \Plawof{1}_{\alg(1)}}\Psi\left(\TVof{\Plawof{1}(\mustar \in \cdot \mid \traj_{t}),\Plawof{2}(\mustar \in \cdot \mid \traj_{t})}\right) \\
&\le \sum_{t=0}^{H-1}\Psi\left(\Expop_{\traj_t \sim \Plawof{1}_{\alg(1)}}\TVof{\Plawof{1}(\mustar \in \cdot \mid \traj_{t}),\Plawof{2}(\mustar \in \cdot \mid \traj_{t})}\right),
%&\le \sum_{t=0}^{H-1}\Psi\left(\Expop_{\traj_t \sim \Plawof{1}}\TVof{\Plawof{1}(\mustar \on \cdot \mid \traj_{t-1}),\Plawof{2}_{t}(\mustar \in \cdot \mid \traj_{t-1})}\right)
\end{align*}
Next, let $\muhat_{t}$ be a random-variable jointly distributed with $\traj_t$ so that, for $i \in \{1,2\}$, $\Plawof{i}_t(\muhat_t \in \cdot \mid \traj_t) = \Plawof{2}_t(\mustar \in \cdot \mid \traj_t)$. Then, 
\begin{align}
&\Expop_{\traj_t \sim \Plawof{1}_{\alg(1)}}\TVof{\Plawof{1}(\mustar \in \cdot \mid \traj_{t-1}),\Plawof{2}(\mustar \in \cdot \mid \traj_{t-1})} \\
&= \Expop_{\traj_t \sim \Plawof{1}_{\alg(1)}}\TVof{\Plawof{1}(\mustar \in \cdot \mid \traj_{t-1}),\Plawof{1}_t(\muhat \in \cdot \mid \traj_{t-1})}\\
&\quad= \TVof{\Plawof{1}_{\alg(1)}(\mustar,\traj_t),\Plawof{1}_{t}(\muhat_t,\traj_t)} \\
%\TVof{\Plawof{1}_{\alg(1)}(\mustar,\traj_{,\Plawof{1}_{t}}\\
&\quad\le \underbrace{\TVof{\Plawof{1}_{\alg(1)}(\mustar,\traj_t),\Plawof{2}_{t}(\muhat_t,\traj_t)}}_{(a)} + \underbrace{\TVof{\Plawof{1}_{t}(\muhat_t,\traj_t),\Plawof{2}_{t}(\muhat_t,\traj_t)}}_{(b)}.
\end{align}
Below, we show that 
\begin{align}
(a) = \TVof{\prior(\theta_1),\prior(\theta_2)}, \quad (b) \le\TVof{\prior(\theta_1),\prior(\theta_2)} \label{eq:a_b_bound}
\end{align} 
Together this yields a bound
\begin{align}
\TVof{\Plawof{1}_{\alg(1)}(\signal_H),\Plawof{1}_{\alg(2)}(\signal_H)} \le H\Psi\left(2\TVof{\prior(\theta_1),\prior(\theta_2)}\right)/
\end{align}

\subsubsection{Proof of \Cref{eq:a_b_bound}}

To bound terms $(a)$ and $(b)$, we invoke the following claim:
\begin{claim}\label{claim:mu_claim}
For $i \in \{1,2\}$ $\Plawof{1}_{\alg(1)}(\traj_t \in \cdot \mid \mustar) = \Plawof{i}_{t}(\traj_t \in \cdot \mid \mustar) = \Plawof{1}_{t}(\traj_t \in \cdot \mid \mustar)$ and $2$.
\end{claim}
This claim holds because the algorithm $\Plawof{1}_{\alg(1)}$ and the algorithm in $\Plawof{2}_{t}$ coincide for times $h=1,2,\dots,t$, and hence the trajectories are the same whenever the realized parameter is. We also use
\begin{claim}\label{claim:TV}
Let $\Plaw,\Qlaw$ be laws over joint random variables $(X,Y)$, such that $\Plaw(Y \in \cdot \mid X ) = \Qlaw(Y \in \cdot \mid X)$. Then, $\TVof{\Plaw(X,Y),\Qlaw(X,Y)} = \TVof{\Plaw(X),\Qlaw(X)}$.
\end{claim}

\paragraph{Term (a)} First, note that use that $\Plawof{2}_{t}(\muhat_t,\traj_t) = \Plawof{2}_{t}(\mustar,\traj_t)$ by construction of the conditional distribution of $\mustar$. Thus, $(a) = \TVof{\Plawof{1}_{\alg(1)}(\mustar,\traj_t),\Plawof{2}_{t}(\mustar,\traj_t)}$. By \Cref{claim:mu_claim} and \Cref{claim:TV}, $ \TVof{\Plawof{1}_{\alg(1)}(\mustar,\traj_t),\Plawof{2}_{t}(\mustar,\traj_t)} =  \TVof{\Plawof{1}_{\alg(1)}(\mustar),\Plawof{2}_{t}(\mustar)}$. Since the marginal laws satisfy $\Plawof{1}_{\alg(1)}(\mustar) = \prior(\theta_1)$ and $\Plawof{2}_{t}(\mustar) = \prior(\theta_2)$, we conclude that $(a) = \TVof{\prior(\theta_1),\prior(\theta_2)}$.

\paragraph{Term (b)}


To bound term $(b)$, we notice that $\Plawof{1}_{t}(\muhat_t \in \cdot \mid \traj_t) = \Plawof{2}_{t}(\muhat_t \in \cdot \mid \traj_t)$ by definition, so  $(b) = \TVof{\Plawof{1}_{t}(\muhat_t,\traj_t),\Plawof{2}_{t}(\muhat_t,\traj_t)} = \TVof{\Plawof{1}_{t}(\traj_t),\Plawof{2}_{t}(\traj_t)}$. Therefore, by data-processing followed by  \Cref{claim:mu_claim} and \Cref{claim:TV},
\begin{align}
(b) &= \TVof{\Plawof{1}_{t}(\traj_t),\Plawof{2}_{t}(\traj_t)} \\
&\le \TVof{\Plawof{1}_{t}(\mustar,\traj_t),\Plawof{2}_{t}(\mustar,\traj_t)}\\
&= \TVof{\Plawof{1}_{t}(\mustar),\Plawof{2}_{t}(\mustar)},
\end{align}
Again, $\Plawof{i}_{t}(\mustar) = \prior(\theta_i)$ for both $ i = 1$ and $i = 2$.
\subsection{Some observations}
\newcommand{\Wlaw}{\mathbb{W}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\Df}{\mathrm{D}_f}
\newcommand{\Dfof}[1]{\mathrm{D}_f(#1)}



 We say that $\alg$ is $(\Psi,\Df)$ Bayesian if
\begin{align*}
\TVof{\Plaw_{\alg(\theta)}(a_t = \cdot \mid \traj_{t-1}), \Plaw_{\alg(\theta')}(a_t = \cdot \mid \traj_{t-1})} \le \Psi(\Dfof{\Plawof{\theta}[\mustar \in \cdot \mid \traj_{t-1}), \Plawof{\theta'}[\mustar \in \cdot \mid \traj_{t-1}]} 
\end{align*}

\begin{example}
\begin{align*}
\TVof{\Plaw_{\alg(\theta)}(a_t = \cdot \mid \traj_{t-1}), \Plaw_{\alg(\theta')}(a_t = \cdot \mid \traj_{t-1})} &\overset{(\text{Pinsker})}{\le} \sqrt{2 \KLof{\Plaw_{\alg(\theta)}(a_t = \cdot \mid \traj_{t-1}), \Plaw_{\alg(\theta')}(a_t = \cdot \mid \traj_{t-1})} }\\
&\overset{(i)}{\le} \sqrt{2 \KLof{\E_{\alg(\theta)}[\mustar  \mid \traj_{t-1}), \E_{\alg(\theta')}[\mustar \mid \traj_{t-1})} }\\
&\overset{(ii)}{\le} \sqrt{2\KLof{\Plawof{\theta}[\mustar \in \cdot \mid \traj_{t-1}), \Plawof{\theta'}[\mustar \in \cdot \mid \traj_{t-1}]}}
\end{align*}
\end{example}
\begin{theorem} Let $\Df$ be an $f$-divergence, where $f$ denotes either total variation, $\chi^2$, hellinger, or $\KL$. Let $\Psi$ be increasing and concave, and let $\alg(\cdot)$ be a family of $(\Psi,\Df)$-Bayesian algorithms over parameters $\theta \in \Theta$, then
\begin{align*}
\TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)} \le H\Psi\left(c_f\Dfof{\prior(\theta),\prior(\theta')}\right),
\end{align*}
where we can take $c_f = 1$ for $\KL$, $c_f = 2$ for $\TV$ and Helinger.
\end{theorem}
\begin{proof} 
\begin{definition}We say that $\Df$ satisfies the \emph{decoupling property} with parameters  $c_{f_1}$ and $c_{f,2}$ if, for  any three laws $\Plaw,\Qlaw,\Wlaw$ be laws over abstract random variables $(X,Y)$ such that (a) $\Plaw[X \in \cdot] = \Qlaw[X \in \cdot]$ are identical, and (b) $\Qlaw[Y \in \cdot \mid X]$ and $\Wlaw[Y \in \cdot \mid X]$ coincide, we have
\begin{align*}
\Dfof{\Plaw(X,Y),\Qlaw(X,Y)} \le c_{f,1}\Dfof{\Plaw(X,Y),\Wlaw(X,Y)} + c_{f,2}\Dfof{\Qlaw(X,Y),\Wlaw(X,Y)} 
\end{align*}
\end{definition}
We first show that if $\Df$ satisfies the \emph{decoupling property} with parameters $c_{f,1}$ and $c_{f,2}$, then for $c_f = c_{f,1} + c_{f,2}$.
\begin{align*}
\TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)} \le H\Psi\left(c_f\Dfof{\prior(\theta),\prior(\theta')}\right),
\end{align*}
Just as for total variation, we have
\begin{align*}
\TVof{\Plawof{1}_{\alg(1)}(\traj_H),\Plawof{1}_{\alg(2)}(\traj_H)}
&\le \sum_{t=0}^{H-1}\Psi\left(\Expop_{\traj_t \sim \Plawof{1}_{\alg(1)}}\Dfof{\Plawof{1}(\mustar \in \cdot \mid \traj_{t}),\Plawof{2}(\mustar \in \cdot \mid \traj_{t})}\right)\\
&= \sum_{t=0}^{H-1}\Psi\left(\Dfof{\Plawof{1}(\mustar, \traj_{t}),\Plawof{1}_t(\mustar,\traj_{t})}\right),
%&\le \sum_{t=0}^{H-1}\Psi\left(\Expop_{\traj_t \sim \Plawof{1}}\TVof{\Plawof{1}(\mustar \on \cdot \mid \traj_{t-1}),\Plawof{2}_{t}(\mustar \in \cdot \mid \traj_{t-1})}\right)
\end{align*}
where the last line remains true for arbitrary $f$ divergences. We now use the decoupling property to bouund
\begin{align*}
\Dfof{\Plawof{1}(\mustar, \traj_{t}),\Plawof{1}_t(\mustar,\traj_{t})} \le c_{1,f}\Dfof{\Plawof{1}(\mustar, \traj_{t}),\Plawof{2}_t(\mustar,\traj_{t})} + c_{2,f}\Dfof{\Plawof{1}_t(\mustar, \traj_{t}),\Plawof{2})t(\mustar,\traj_{t})}.
\end{align*}
The same data-processing and distributionc haracterization arguments apply, so $\Dfof{\Plawof{1}(\mustar, \traj_{t}),\Plawof{2}_t(\mustar,\traj_{t})} = \Dfof{\pi(\theta_1),\pi(\theta_2)}$, and $\Dfof{\Plawof{1}_t(\mustar, \traj_{t}),\Plawof{2})t(\mustar,\traj_{t})} = \Dfof{\Plawof{1}_t(\traj_{t}),\Plawof{2}_t(\traj_{t})} \le \Dfof{\pi(\theta_1),\pi(\theta_2)}$. This yields
\begin{align*}
\Dfof{\Plawof{1}(\mustar, \traj_{t}),\Plawof{1}_t(\mustar,\traj_{t})} \le \underbrace{(c_{1,f}+ c_{2,f})}_{:=c_f}\Dfof{\pi(\theta_1),\pi(\theta_2)}, 
\end{align*}
and the bound follows. To conclude, we bound the decoupling constants.
\begin{lemma} Decoupling constants for the various $f$-divergences are bounded as follows:
\begin{itemize}
	\item $c_{f,1},c_{f,2} = 1$ for Hellinger and Total Variation.
	\item $c_{f,1} = 1$, $c_{f,2} = 0$ for $\KL$. 
		\end{itemize}
\end{lemma}

\begin{proof}
The first item follows since total variation and Hellinger are metrics in the space of probability measures, and therefore satisfy the triangle inequality. For the $\KL$ inequality,
\begin{align*}
\KL(\Plaw(X,Y),\Qlaw(X,Y)) &= \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Plaw(x,y)}{\rmd \Qlaw(x,y)}\\
&= \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Plaw(x,y)}{\rmd \Wlaw(x,y)} + \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Wlaw(x,y)}{\rmd \Qlaw(x,y)}\\
&= \KL(\Plaw(X,Y),\Wlaw(X,Y)) + \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Wlaw(x,y)}{\rmd \Qlaw(x,y)}
\end{align*}
Now, since $\Qlaw[Y \in \cdot \mid X]$ and $\Wlaw[Y \in \cdot \mid X]$ coincide, we have 
\begin{align*}
 \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Wlaw(x,y)}{\rmd \Qlaw(x,y)} &=  \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Wlaw(x)}{\rmd \Qlaw(x)} = \int_{x}\rmd \Plaw(x) \log \frac{\rmd \Wlaw(x)}{\rmd \Qlaw(x)}.
\end{align*}
Moreover, since $\rmd\Plaw(x) = \rmd\Qlaw(x)$, we conclude that
\begin{align*}
 \int_{(x,y)}\rmd \Plaw(x,y) \log \frac{\rmd \Wlaw(x,y)}{\rmd \Qlaw(x,y)} = \int_{x}\rmd \Qlaw(x) \log \frac{\rmd \Wlaw(x)}{\rmd \Qlaw(x)} = -\KL(\Qlaw,\Wlaw) \le 0.
\end{align*}
\end{proof}
\begin{comment}
The argument for the $\chi^2$ divergence is slightly different. We have
\begin{align*}
\chi^2_N(\Plaw(x,y),\Qlaw(x,y)) &= \int_{(x,y)} \frac{(\rmd\Qlaw(x,y)-\rmd\Plaw(x,y))^2}{\rmd \Plaw(x,y)}\\
&= 2\int_{(x,y)} \frac{(\rmd\Wlaw(x,y)-\rmd\Plaw(x,y))^2}{\rmd \Plaw(x,y)} + 2\int_{(x,y)} \frac{(\rmd\Qlaw(x,y)-\rmd\Wlaw(x,y))^2}{\rmd \Plaw(x,y)}\\
&= 2\chi^2_N + 2\int_{(x,y)} \frac{(\rmd\Qlaw(x,y)-\rmd\Wlaw(x,y))^2}{\rmd \Plaw(x,y)}\\
&= 2\chi^2_N + 2\int_{x} \frac{\rmd \Qlaw(y \mid x) (\rmd\Qlaw(x)-\rmd\Wlaw(x))^2}{\rmd \Plaw(x)\rmd \Plaw(y \mid x)}\\
&= 2\chi^2_N + 2\int_{x} \frac{(\rmd \Qlaw(y \mid x))^2 (\rmd\Qlaw(x)-\rmd\Wlaw(x))^2}{\rmd \Plaw(x)\rmd \Plaw(y \mid x)}\\
&= 2\chi^2_N + 2\int_{x} \frac{(\rmd\Qlaw(x)-\rmd\Wlaw(x))^2}{\rmd \Plaw(x)} \int_{y}\frac{(\rmd \Qlaw(y \mid x))^2}{\rmd \Plaw(y \mid x)}.
\end{align*}
Now, we have
x
\end{comment}
\end{proof}

\subsection{A lower bound}

Here we show that, up to constant factors, the dependence on $H$ and $n$ in the upper bounds are unavoidable for general $n$-Monte Carlo Bayesian algorithm. To do this, consider the following $n$-Monte Carlo Bayesian algorithm that generalizes Thompson sampling.
\begin{itemize}
	\item[] At each time step $t$:
	\begin{itemize}[label=$\bullet$]
		\item Draw $\mu^{(1)}, \ldots, \mu^{(n)}$ from the current posterior. %$\Plawof{\theta}(\mustar \in \cdot \mid \traj_t)$.
		\item For each coordinate $k$, let $v_k = \max\{ \mu^{(1)}_k, \ldots, \mu^{(n)}_k\}$. 
		\item Choose the arm $k^* = \argmax_{k} v_k$. If there are multiple such arms, then pull one arbitrarily.
	\end{itemize}
\end{itemize}
Let $\alg(\theta)$ denote this algorithm with prior $\pi(\theta)$. Consider the following two prior distributions. 
\begin{itemize}
	\item $\pi(\theta)$ places all its probability mass on the vector $(1/2, 0)$.
	\item $\pi(\theta')$ places $1-\epsilon$ of its probability mass on the vector $(1/2, 0)$ and $\epsilon$ of its probability mass on the vector $(1/2, 1)$.
\end{itemize}
Clearly we have $\TVof{\pi(\theta), \pi(\theta')} = \epsilon$. We will give a lower bound on $\TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)}$. To do so, we make three observations.
\begin{itemize}
	\item[(a)] $\alg(\theta)$ will always pull arm 1. Thus, to give a lower bound on the total variation distance between the behavior of $\alg(\theta)$ and $\alg(\theta')$, it suffices to lower bound the probability that $\alg(\theta')$ pulls arm $2$ in the course of $H$ interactions.
	\item[(b)] The posterior distribution under $\theta'$ remains unchanged when arm 1 is pulled. Thus, the probability that $\alg(\theta')$ never pulls arm $2$ in the course of $H$ interactions is the $H$-fold product of the probability that $\alg(\theta')$ does not pull arm 2 in one round of interaction.
	\item[(c)] The probability that $\alg(\theta')$ does not pull arm 2 in one round of interaction is exactly the probability that $n$ i.i.d. draws from $\theta'$ does not yield an instance of $(1/2, 1)$, i.e. $(1-\epsilon)^n$. 
\end{itemize}
Combining (a), (b), and (c), and assuming $\epsilon \leq \frac{1}{2Hn}$,
\begin{align*}
\TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)} 
\geq 1 - (1-\epsilon)^{Hn} 
\geq 1 - e^{-\epsilon H n} 
\geq \epsilon H n - (\epsilon H n)^2 \geq \frac{1}{2} \epsilon H n.
\end{align*}
In the above we have used the inequality $e^{-x} \leq 1 - x+ x^2$ for $x \in [0,1]$ and the assumption that $\epsilon \leq \frac{1}{2Hn}$. Recalling that $\TVof{\pi(\theta), \pi(\theta')} = \epsilon$, we have an example where 
\[ \TVof{\Plawof{\theta}_{\alg(\theta)}(\traj_H),\Plawof{\theta}_{\alg(\theta')}(\traj_H)}  \ \geq \ \frac{H n}{2} \TVof{\pi(\theta), \pi(\theta')} .  \]

\begin{comment}
Alternative notation:
\begin{itemize}
    \item $P^\theta_t$ the law when the truth is $\theta$ and the algorithm switches from $\TS_{\theta_1}$ to $\TS_{\theta_2}$ in step $t$.
    \item $P^\theta_t( (H_{1:t}, a_{t+1}) )$
    \item $P_{H+1}^\theta$ is the law when the truth is $\theta$ and the algorithm is just $\TS_{\theta_1}$.
    \item $P_{\star}^\theta$: the truth $\theta$ and the algorithm is $\theta$.
    \item $\TV(P^\theta(x_{1:t})$
    \item $P^{\theta}_{\alg(\theta')}$ for theorem
    \item $)$
    \item $\signal_h =$
\end{itemize}
\begin{align*}
    \forall H \in \N,\quad \TVof{\Plaw^{\theta_1}_{\alg(\theta_1)}(\traj_{H}), \Plaw^{\theta_1}_{\alg(\theta_2)}(\traj_{H})} %= \TVof{P^{\theta_1}_{\alg(\theta_1)}(\signal_{H}), P^{\theta_1}_{\alg(\theta_2)}(\signal_{H})} 
    \le 6H\TVof{\pi(\theta_1),\pi(\theta_2)}
\end{align*}

Let us define the following random variables:


Let $\TS_{\theta}$ denote running pure Thompson sampling with prior $\pi(\theta)$, and let $\TS_{\theta_1,\theta_2;t}$ denote the algorithm which rolls in Thompson-sampling under $\theta_1$ for $t$-steps, and rollouts out Thompson-sampling under $\theta_2$. Given an algorithm $\alg$, let $\Law_{\theta,t}(\alg)$ denote the law of all actions generated by the algorithm from time steps $1,2,\dots,t$ and rewards from times $1,2,\dots,t-1$ under $\mu$ being drawn from the prior $\theta$.


Given jointly distributed random variables (with possibly different domains) $(\matx_1,\matx_2,\dots)$, we let $\matx_{s:t}$ denote the system $(\matx_s,\matx_{s+1},\dots,\matx_t)$. 




\begin{theorem} For any parameters $\theta_1,\theta_2$, and 
\begin{align*}
\TVof{\Law_{\theta_1,H}(\TS_{\theta_1}),\Law_{\theta_1,H}(\TS_{\theta_2})} \le 4H\TVof{\pi(\theta_1),\pi(\theta_2)}
\end{align*}
\end{theorem}
\begin{proof}
By the triangle inequality/performance difference,
\begin{align}
\TV(\Law_{\theta_1;H}(\TS_{\theta_1}),\Law_{\theta_1;H}(\TS_{\theta_2})) \le \sum_{h=0}^{H-1}\TVof{\Law_{\theta_1,h+1}(\TS_{\theta_1,\theta_2;h}),\Law_{\theta_1,h+1}(\TS_{\theta_1})} \label{eq:b_decomp},
\end{align}
\akcomment{The naive triangle inequality bound is
\begin{align*}
\TV(\Law_{\theta_1;H}(\TS_{\theta_1}),\Law_{\theta_1;H}(\TS_{\theta_2})) \le \sum_{h=0}^{H-1}\TVof{\Law_{\theta_1,H}(\TS_{\theta_1,\theta_2;h}),\Law_{\theta_1,H}(\TS_{\theta_1,\theta_2;h+1})}.    
\end{align*}
How do you go from here to the expression above? (The difference is whether you are looking at the law of all $H$ actions or just the first $h+1$.) I guess there is a data processing inequality or something: If the action at time $h+1$ is the same, then the two distributions are identical. But let's explain this part carefully.
}
that is, we decompose the total TV into the TV between algorithms which switch from $\theta_1$-$\TS$ to $\theta_2$-TS. Now, we bound the term in the sum:
\begin{equation}\label{eq:a_decomp}
\begin{aligned}
&\TVof{\Law_{\theta_1,t+1}(\TS_{\theta_1,\theta_2;t}),\Law_{\theta_1,t+1}(\TS_{\theta_1})} \\
&\le \TVof{\Law_{\theta_2,t+1}(\TS_{\theta_1,\theta_2;t}),\Law_{\theta_1,t+1}(\TS_{\theta_1})}\\
&\quad + \TVof{\Law_{\theta_1,t+1}(\TS_{\theta_1,\theta_2;t}),\Law_{\theta_2,t+1}(\TS_{\theta_1,\theta_2;t})}\\
&\le \TVof{\Law_{\theta_2,t+1}(\TS_{\theta_1,\theta_2;t}),\Law_{\theta_1,t+1}(\TS_{\theta_1})}+ \TVof{\pi(\theta_1),\pi(\theta_2)}.
\end{aligned}
\end{equation}
\akcomment{The first inequality is the triangle inequality, and the second is by data processing. In particular, we are running exactly the same algorithm, namely $\TS_{\theta_1,\theta_2;t}$, on two different priors.}

Adopt the shorthand $\Law_2 := \Law_{\theta_2,t+1}(\TS_{\theta_1,\theta_2;t})$ and $\Law_1 := \Law_{\theta_1,t+1}(\TS_{\theta_1})$. Under each $\Law_i$, the true rewards are drawn with $\mu_{\star;i}$ drawn from $\pi(\theta_i)$. Moreover, the policy for arm selects coincide for times $s = 1,2,\dots,t$, but differ at time $t+1$. In particular, letting $\Hcal_{t;i}$ denote this history of actions and rewards, we see  $\Hcal_{t;i} \mid \mu_{\star;i}$ is the same for $i = 1,2$ \akedit{although the distribution of $\mu_{\star,i}$ is not the same for $i=1,2$}. Finally, the action selected at time $t+1$ is a function of a hallucinated posterior $\muhat_{t+1;i}$. Since the rewards in $\Law_i$ are drawn from $\mu_{\star;i} \sim \pi(\theta_i)$, the posteriors are valid, and hence 
\begin{align*}
\mu_{\star;i}, \muhat_{t+1;i} \text{ are i.i.d. } \mid \Hcal_{t;i}, \quad i = 1,2.
\end{align*}
\akcomment{Of course, $\mu_{\star,1}$ and $\muhat_{t,2}$ are independent, but not identically distributed given $\Hcal_{t,i}$.}

Note that $\Law_i$ is entirely specified by the triple $(\mu_{\star;i},\muhat_{t+1;i},\Hcal_{t;i})$. Hence, we can apply the following lemma;

\begin{lemma}\label{lem:structured_TV_comp}
Consider two sets of random variables $W_1 = (\mu_1,\muhat_1,\traj_1)$ and $W_2 = (\mu_2,\muhat_2,\traj_2)$. Suppose that
\begin{itemize} 
    \item For $i \in \{1,2\}$ for $\mu^i,\muhat^i $ are i.i.d given $\traj_i$. 
\item The conditional distributions of $\traj$ given $\mu$ are identical: $\Pr[\traj_1 \in \cdot \mid \mu_1 ] = \Pr[\traj_2\in \cdot \mid \mu_2 ]$
\end{itemize}
Then, $\TVof{W_1,W_2} \le 5\TVof{\mu_1,\mu_2}$.
\end{lemma}
By the above lemma, we find
\begin{align*}
\TVof{\Law_{2},\Law_{1}} \le 5\TVof{\mu_{\star,1},\mu_{\star,2}} = 5\TVof{\pi(\theta_1),\pi(\theta_2)}
\end{align*}
Hence \Cref{eq:a_decomp} implies
\begin{align*}
\TVof{\Law_{\theta_1,t+1}(\TS_{\theta_1,\theta_2;t}),\Law_{\theta_1,t+1}(\TS_{\theta_1,\theta_2;t+1})} \le 6\TVof{\pi(\theta_1),\pi(\theta_2)}
\end{align*}
and hence, \Cref{eq:b_decomp} yields
\begin{align*}
\TVof{\Law_{\theta_1;H}(\TS_{\theta_1}),\Law_{\theta_1;H}(\TS_{\theta_1,\theta_2})} \le 6H\TVof{\pi(\theta_1),\pi(\theta_2)}
\end{align*}
\end{proof}


\begin{proof}[Proof of\Cref{lem:structured_TV_comp}] We construct an interpolating distribution $Z_3 = (X_3,\Xtil_3,Y_3)$, such that $Y_3$ has the same marginal distribution as $Y_1$, and $X_3,\Xtil_3 \mid Y_3$ have the same conditional distribution as $X_2,\Xtil_2 \mid Y_2$. By the triangle inequality and symmetry of total variation, $\TVof{Z_1,Z_2} \le \TVof{Z_2,Z_3} + \TVof{Z_1,Z_3}$. Bounding the first term is straightforward
\begin{align*}
\TVof{Z_2,Z_3} &= \TVof{Y_1,Y_3} = \TVof{Y_1,Y_2} \le \TVof{X_1,Y_1;X_2,Y_2}.
\end{align*}
To bound the second term, let $\P_{Y_1}$ denote the marginal law of $Y_1$. Then 
\begin{align*}
\TVof{Z_1,Z_3} &= \E_{Y \sim \P_{Y_1} }[\TVof{(X_1,\Xtil_1) \mid Y_1 = Y; (X_3,\Xtil_3) \mid Y_3 = Y}]\\
&\le 2\E_{Y \sim \P_{Y_1} }\TVof{X_1 \mid Y_1 = Y; X_3 \mid Y_3 = Y}]\\
&= 2\TVof({X_1,Y_1);(X_3,Y_3)}\\
&= 2\TVof{(X_1,Y_1);(X_2,Y_2)}
\end{align*}
Therefore, by the triangle inequality, $\TVof{\akedit{Z_1,Z_2}} \le 3\TVof{(X_1,Y_1);(X_2,Y_2)}$. Finally, since $Y_1 \mid X_1$ and $Y_2 \mid X_2$ are identically distributed, $\TVof{(X_1,Y_1);(X_2,Y_2)} = \akedit{ \TVof{X_1;X_2}}$.
\end{proof}

\akcomment{I think the last part is not quite correct. Here is my argument. As above we start with
\begin{align*}
    \TVof{Z_1; Z_2} \leq 2 \TVof{(X_1, Y_1); (X_3, Y_3)}.
\end{align*}
Now, we can write
\begin{align*}
    \TVof{(X_1, Y_1); (X_3, Y_3)} &= \frac{1}{2} \int | p_1(x\mid y) p_1(y) - p_3(x\mid y) p_3(y) | \\
    & = \frac{1}{2} \int | p_1(x\mid y) p_1(y) - p_2(x\mid y) p_1(y) |\\
    & \leq \frac{1}{2}\int |p_1(x\mid y)p_1(y) - p_2(x\mid y) p_2(y)| + \frac{1}{2}\int |p_2(x\mid y)p_1(y) - p_2(x\mid y) p_2(y)|\\
    & = \TVof{(X_1,Y_1); (X_2, Y_2)} + \TVof{Y_1; Y_2}\\
    & \leq 2 \TVof{(X_1,Y_1); (X_2, Y_2)}
\end{align*}
Maybe I'm being slow, but for the last inequality, observe that
\begin{align*}
    \TVof{Y_1;Y_2} = \sup_{A \subset\mathcal{Y}} |P_1(A) - P_2(A)| \leq \sup_{B \subset \mathcal{X}\times\mathcal{Y}} |P_1(B) - P_2(B)|,
\end{align*}
where the inequality holds since we can take $B = \mathcal{X} 
\times A^\star$ where $A^\star$ is the maximizer of the first supremum (and use the fact that the distribution integrates to $1$). Using this above, I think we end up with a constant of $5$. 



}\end{comment}

\begin{comment}
\section{Basic smoothness observations}
Let $P$ be the true prior.  In the explore then commit strategy we
will learn a prior $\hat{P}$ and we will use $\hat{P}$ as an argument
to our algorithm $\alg$ (e.g., Thompson sampling). We want to say that
running $\alg(\hat{P})$ on a Bayesian bandit problem with true prior
$P$ will not be too bad. This requires showing some kind of smoothness.

The basic observation is that for any algorithm $\alg$, we have
\begin{align}
& \left| \En_{\theta \sim P}\left[ \reg(T,\alg,\theta)\right]  - \En_{\theta \sim \hat{P}}\left[ \reg(T,\alg,\theta)\right] \right| \\
& = \left| \int \reg(T,\alg,\theta) (dP(\theta) - d\hat{P}(\theta)) \right|\\
& \leq \int \one\{\|\mu(\theta)\|_{\infty} \leq B\} | \reg(T,\alg,\theta) | \cdot |dP(\theta) - d\hat{P}(\theta)| + \int \one\{\|\mu(\theta)\|_{\infty} > B\} |\reg(T,\alg,\theta)| \cdot |dP(\theta) - d\hat{P}(\theta)| \\
& \leq O(BT) \| P - \hat{P} \|_{\mathrm{TV}} + \int \one\{\|\mu(\theta)\|_{\infty} > B\} |\reg(T,\alg,\theta)| \cdot |dP(\theta) - d\hat{P}(\theta)|.
\end{align}
If the model is such that for any $P \in \mathcal{P}$, with
probability 1 we have $\| \mu(\theta) \|_{\infty} \leq B$, then we are
done here. Otherwise we will have to bound this ``tail mean'', which
seems do-able for models with favorable tails.

Now we do the ERM computation. Let us assume that 
\begin{align}
P = \argmin_{\tilde{P} \in \mathcal{P}} \En_{\theta \sim P}\left[ \reg(T,\alg(\tilde{P}), \theta)\right].
\end{align}
This just means that, if the true prior is $P$ then the best algorithm
parameter to use is $P$ itself. If this is true, then
\begin{align}
\En_{\theta \sim P^\star}\left[\reg(T,\alg(\hat{P}),\theta)\right] &\leq \Delta(P^\star,\hat{P}) + \En_{\theta \sim \hat{P}}\left[\reg(T,\alg(\hat{P}),\theta)\right]\\
& \leq \Delta(P^\star,\hat{P}) + \En_{\theta \sim \hat{P}}\left[\reg(T,\alg(P^\star),\theta)\right]\\
& 2 \Delta(P^\star,\hat{P}) + \En_{\theta \sim P^\star }\left[\reg(T,\alg(P^\star),\theta)\right]
\end{align}
Here $\Delta$ is the ``uniform smoothness'' that we can ideally
establish. For example in the bounded mean case, we can take
$\Delta(P_1,P_2) = O(BT)\|P_1 - P_2\|_{\mathrm{TV}}$. 

\begin{remark}
Note that this would work fine if we simply \emph{define} $\alg(P)$ to
be the best configuration of our base learner for prior $P$. In
general the best configuration may not be $P$ itself.
\end{remark}


\section{Refined smoothness for Thompson Sampling}

We can define $\TS(\theta_1;\theta_0)$ as the following stochastic process:
\newcommand{\posterior}{\mathrm{post}}
\begin{align*}
    \mu &\sim \theta_0\\
    z_{t,a} &~ \posterior_t(\cdot \mid \theta_1)\\
    a_t &\sim \argmax_{a} z_{t,a}\\
    X_{t} & \sim \mathcal{N}(\mu[a_t],1)
\end{align*}



\begin{align*}
    \mathcal{H}_0 = \emptyset, \quad \vec{\mu}_0 \sim \theta_0 \\
    \vec{z}_{t} \sim p_t(\cdot \mid \mathcal{H}_{t-1}, \theta_1)\\
    a_t \sim \argmax_{a} z_t(a)\\
    r_t \sim \mathcal{N}(\mu_0(a_t), 1)\\
    \mathcal{H}_{t} \gets \mathcal{H}_{t-1} \cup \{a_t,r_t\}
\end{align*}


\begin{align*}
    \mathcal{H}_0 = \emptyset,  \\
    \zrew_{t,\thetast} \sim p_t(\cdot \mid \Hcal_{t-1},\thetast)\\
    \zts_{t,\thetahat} \sim p_t(\cdot \mid \Hcal_{t-1},\thetahat)\\
    \zts_{t,\thetast} \sim p_t(\cdot \mid \Hcal_{t-1},\thetast)\\
    \ats_{t,\thetahat} = \argmax_{a} \zts_{t,\thetahat}(a)\\
    \ats_{t,\thetast} = \argmax_{a} \zts_{t,\thetast}(a)\\
    a_{t} = \ats_{t,\thetast} \\
    r_{t,\thetahat} \sim \mathcal{N}(\zrew_{t,\thetast}(a_t), 1)\\
    \mathcal{H}_{t} \gets \mathcal{H}_{t-1} \cup \{a_t,r_t\}
\end{align*}
Under some expectation, what is
\begin{align*}
    \TV(\Law(\TS(\thetahat;\thetast));\Law(\TS(\thetast;\thetast))) \le \inf_{\text{couplings }  (\zts_{t,\thetahat} ,  \zts_{t,\thetast}) }\sum_{t=1}^H \Pr[ \ats_{t,\thetast} \ne \ats_{t,\thetahat} ] \le H \TV(\Law(\thetast),\Law(\thetahat))
\end{align*}


\begin{align*}
    \KL(\Law(\TS(\thetahat;\thetast));\Law(\TS(\thetast;\thetast))) = \sum_{t=1}^H   \E_{\thetahat; \thetast}\KL(\ats_{t,\thetahat} ;\ats_{t,\thetast} )
\end{align*}
\begin{align*}
    \KL(\ats_{t,\thetahat} ;\ats_{t,\thetast} ) \le \KL(\zts_{t,\thetahat} ;\zts_{t,\thetast} )
\end{align*}
\subsection{Some Stuff}
\newcommand{\pulls}{\mathsf{pulls}}
\newcommand{\Ppult}[1][t]{\Pr_{\mathrm{pul},t}}
\newcommand{\Prewt}[1][t]{\Pr_{\mathrm{rew},t}}
\newcommand{\Ppost}{\Pr_{\mathrm{post}}}

\newcommand{\rews}{\mathsf{rews}}

\end{comment}


==> preamble/packages-neurips.tex <==
%!TEX root = ../main.tex


\usepackage{amsthm,etoolbox}
  \usepackage{inconsolata}

\newtoggle{neurips}
\toggletrue{neurips}

% DeclarePairedDelimiter
\usepackage{mathtools}
%\usepackage{bbold}
% DeclareMathOperator
\usepackage{amsmath}

% mathbbm
\usepackage{amsfonts}
\usepackage{bbm}

% triangleq
\usepackage{amssymb}

% rrangle, llangle
%\usepackage{MnSymbol} %Actually conflicts with amssymb and others
%apparently. Doesn't work with pxfonts either.

% fancy
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

%\usepackage[noend]{algpseudocode}
%\usepackage[linesnumbered,noend, ruled]{algorithm2e}
%\usepackage[letterpaper, left=1in, right=1in, top=1in,bottom=1in]{geometry}

\usepackage{verbatim}

\usepackage{booktabs} % For formal tables

\usepackage[utf8]{inputenc}

\usepackage{geometry}


\usepackage{graphpap,amscd,mathrsfs,graphicx,lscape,enumitem,dsfont,bm,url,subfigure}
\usepackage{epsfig,amstext,xspace}

\usepackage{thmtools,thm-restate}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{bbm}
\usepackage{cleveref}

\usepackage{microtype} 

% tikz
\usepackage{tikz}
\usetikzlibrary{intersections}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{matrix}
\usetikzlibrary{calc}


\newif\ifpx
\DeclareOption{px}{\pxtrue}

\ProcessOptions

\ifpx
  \let\iint\relax
  \let\iiint\relax
  \let\iiint\relax
  \let\idotsint\relax
  \usepackage[varg]{pxfonts}
\fi

\usepackage{enumitem}
\setlist{leftmargin=0.5cm,itemsep=2pt,parsep=0pt}
